Parameterized Approximation for Capacitated $d$-Hitting Set with Hard Capacities

The \textsc{Capacitated $d$-Hitting Set} problem involves a universe $U$ with a capacity function $\mathsf{cap}: U \rightarrow \mathbb{N}$ and a collection $\mathcal{A}$ of subsets of $U$, each of size at most $d$. The goal is to find a minimum subset $S \subseteq U$ and an assignment $\phi : \mathcal{A} \rightarrow S$ such that for every $A \in \mathcal{A}$, $\phi(A) \in A$, and for each $x \in U$, $|\phi^{-1}(x)| \leq \mathsf{cap}(x)$. For $d=2$, this is known as \textsc{Capacitated Vertex Cover}. In the weighted variant, each element of $U$ has a positive integer weight, with the objective of finding a minimum-weight capacitated hitting set. Chuzhoy and Naor [SICOMP 2006] provided a factor-3 approximation for \textsc{Capacitated Vertex Cover} and showed that the weighted case lacks an $o(\log n)$-approximation unless $P=NP$. Kao and Wong [SODA 2017] later independently achieved a $d$-approximation for \textsc{Capacitated $d$-Hitting Set}, with no $d - \epsilon$ improvements possible under the Unique Games Conjecture. Our main result is a parameterized approximation algorithm with runtime $\left(\frac{k}{\epsilon}\right)^k 2^{k^{O(kd)}}(|U|+|\mathcal{A}|)^{O(1)}$ that either concludes no solution of size $\leq k$ exists or finds $S$ of size $\leq 4/3 \cdot k$ and weight at most $2+\epsilon$ times the minimum weight for solutions of size $\leq k$. We further show that no FPT-approximation with factor $c > 1$ exists for unweighted \textsc{Capacitated $d$-Hitting Set} with $d \geq 3$, nor with factor $2 - \epsilon$ for the weighted version, assuming the Exponential Time Hypothesis. These results extend to \textsc{Capacitated Vertex Cover} in multigraphs. Additionally, a variant of multi-dimensional \textsc{Knapsack} is shown hard to FPT-approximate within $2 - \epsilon$.

==> abhishek.tex <==
\section{A $\frac{4}{3}$-approximation algorithm}

Consider an instance $(U,\mathsf{cap},\mathcal{A})$ of \textsc{Capacitated $d$-Hitting Set}.


\begin{algorithm}[h]
    \caption{\textsc{CapHS}$(S)$}
    \begin{algorithmic}[1]
        \State $r \leftarrow k-|S|$
        \For{$x \in U \backslash S$}
            \State $\mathsf{color}(x) \leftarrow$ a random number in $[r]$
        \EndFor
        \For{$i=1,\dots,r$}
            \State $C_i \leftarrow \{x \in U \backslash S: \mathsf{color}(x) = i\}$
        \EndFor
        \State $t \leftarrow \lfloor \log_{1+\frac{1}{k}} |\mathcal{A}| \rfloor$ and $S^* \leftarrow U$
        \For{every map $\pi:2^S \rightarrow S$ and every map $\gamma: [r] \times S \rightarrow \{\lceil (1+\frac{1}{k})^p \rceil: p \in [t]\}$}
            \For{$y \in S$}
                \State $\mathcal{A}_y \leftarrow \{A \in \mathcal{A}: \pi(A \cap S) = y\}$
            \EndFor
            \For{$i=1,\dots,r$}
                \State $\delta_i \leftarrow \sum_{y \in S} \gamma(i,y)$
                \State $C_i' \leftarrow \{x \in C_i: \mathsf{cap}(x) \geq \delta_i \text{ and } |\mathcal{A}_y \odot x| \geq \gamma(i,y) \text{ for all } y \in S\}$
            \EndFor
            \If{there exists $i \in [r]$ such that $|C_i'| \leq f(k)$}
                \State $S^* \leftarrow \min\{S^*,\min_{x \in C_i'} \textsc{CapHS}(S \cup \{x\})\}$
            \Else
                \For{$y \in S$}
                    \State $i_y \leftarrow \arg\max_{i \in [r]} \gamma(i,y)$
                    \State $j_y \leftarrow \arg\max_{j \in [r] \backslash \{i_y\}} \gamma(j,y)$
                    \For{$x \in U \backslash S$}
                        \State $i \leftarrow \mathsf{color}(x)$
                        \State $\mathsf{scr}_y(x) \leftarrow \min\{|\mathcal{A}_y \odot x|,\mathsf{cap}(x)-\delta_i+\gamma(i,y)\}$                    
                    \EndFor
                \EndFor
                \For{$i=1,\dots,r$}
                    \State $C_i'' \leftarrow \bigcup_{y \in S: i_y=i} \textsc{Top}(C_i',\mathsf{scr}_y,f(k))$
                \EndFor
                \State $S^* \leftarrow \min\{S^*,\min_{x \in \bigcup_{i=1}^r C_i''} \textsc{CapHS}(S \cup \{x\})\}$
                \State $G \leftarrow \textsc{Bipartite}([r],S,\{(i_y,y): y \in S\} \cup \{(j_y,y): y \in S\})$
                \State $X \leftarrow \{i \in [r]: |\{y \in S: i_y = i\}| \geq 2\}$
                \State Compute a minimum-size $D \subseteq [r]$ satisfying $X \subseteq D$ and $N_G(D) = S$
                \State Compute a subset $R \subseteq \bigcup_{i=1}^r C_i''$ satisfying that
                
                \ \ \ \ \ \ \ \ \ \ $\bullet$ $|R \cap C_i''| = 2$ for $i \in D$
                
                \ \ \ \ \ \ \ \ \ \ $\bullet$ $|R \cap C_i''| = 1$ for $i \in [r] \backslash D$

                \ \ \ \ \ \ \ \ \ \ $\bullet$ $R$ is $\frac{1}{k^2}$-almost $\mathcal{A}_y$-independent for all $y \in S$
                \If{$S \cup R$ is a feasible solution}{ $S^* \leftarrow \min\{S^*,S \cup R\}$}
                \EndIf
            \EndIf
        \EndFor
        \State \textbf{return} $S^*$
    \end{algorithmic}
    \label{alg-caphs}
\end{algorithm}



\section{Auxiliary things}


\subsection{$\rho$-independence}
\todo{define $\rho$-independence definition}
Given a tuple $(S,X=X_1\uplus \cdots \uplus X_{k-|S|},\pi,\gamma)$, to capture the notion of $\rho$-independence among the elements of $X$, we define the auxiliary graphs $H_{(X,\mathcal{A}_s,\rho)}$ $\forall s \in S$ where $V(H_{(X,\mathcal{A}_s,\rho)})=X$. $a$ and $b$ are adjacent in $H_{(X,\mathcal{A}_s,\rho)}$ if the number of sets in $\mathcal{A}_s$ containing both $a$ and $b$ are less than $\rho$ fraction of the number of sets in $\mathcal{A}_s$ containing $a$ as well as less 
less than $\rho$ fraction of the number of sets in $\mathcal{A}_s$ containing $b$. Formally, $(a,b)\in E(H_{(X,\mathcal{A}_s,\rho)})$ if and only if $|(\mathcal{A}_s\odot a) \cap (\mathcal{A}_s\odot b)| > \rho \cdot \text{min}\{|(\mathcal{A}_s\odot a)|, |(\mathcal{A}_s\odot b)|\}$. 

\begin{lemma}\label{degbound}
$\delta(H_{(X,\mathcal{A}_s,\rho)}) \leq d/\rho$.
\end{lemma}

\begin{proof}
 Let $x\in V(H_{(X,\mathcal{A}_s,\rho)})$ be a vertex with degree more than $d/\rho$. From the construction of $H_{(X,\mathcal{A}_s,\rho)}$ $\forall y\in N_{H_{(X,\mathcal{A}_s,\rho)}}(x)$, $|\mathcal{A}_s\odot y\cap |\mathcal{A}_s\odot x|> \rho \cdot |\mathcal{A}_s\odot x|$. Since $\sum_{y\in N_{H_{(X,\mathcal{A}_s,\rho)}}} |\mathcal{A}_s\odot y|\cap |\mathcal{A}_s\odot x|>(d/\rho)\cdot(\rho\cdot |\mathcal{A}_s\odot x|)= d \cdot |\mathcal{A}_s\odot x|$, by pigeonhole principle, there exists a set in $|\mathcal{A}_s\odot x|$ that is present $|A\odot y|$ for $d+1$ many distinct $y$s in $N_{H_{(X,\mathcal{A}_s,\rho)}}(x)$, a contradiction to the fact that any set has at most $d$ elements. Hence the maximum degree of $H_{(X,\mathcal{A}_s,\rho)}$ is $d/\rho$.   
\end{proof}

We define another auxiliary graph $H_{(X,S,\rho)}=(X,E)$ where $E=\{(a,b)| \exists s\in S\text{ s.t. } (a,b)\in H_{(X,\mathcal{A}_s,\rho)} \}$. Two elements $a$ and $b$ are \emph{$\rho$-independent} if and only if they are non-adjacent in $H_{(X,S,\rho)}$. Intuitively two elements $a,b$ in $X$ are $\rho$- independent w.r.t. $S$ if and only if in every $\mathcal{A}_s$, the number of sets containing both $a$ and $b$ are less than $\rho$ fraction of the sets that contain $a$ as well as less than $\rho$ fraction of the sets  containing $b$.
And as an implication of Lemma \ref{degbound} we have the following result. 

\begin{corollary}
$\delta(H_{(X,S,\rho)}) \leq dk/\rho$.
\end{corollary}

\begin{lemma}
Given a tuple $(S,X=X_1\uplus \cdots \uplus X_{k-|S|},\pi,\gamma)$ and a family of disjoint sets $\{Y_i\}_{i=1}^{k-|S|}$, where each $Y_i\subseteq X_i$ of size at least $2(k-|S|)\cdot d/\rho $, there exists a $\rho$- independent set  $O$  such that $|O\cap Y_i|\geq 2$.
\end{lemma}

\begin{proof}
We demonstrate our proof through the inductive construction of the set $O$. We initialize $O_0=\emptyset$. At the $i$th step where $i\in[k-|S|]$, we select 2 vertices from $X_i$ that are non-adjacent in $H_{(X,S,\rho)}$ and have no edges to any vertex in $O_{i-1}$. These vertices are then added to $O_{i-1}$ to form $O_i$, and ultimately, we define $O=O_{k-|S|}$. This is feasible since $\delta(H_{\rho}) \leq dk/\rho$ and $X_i$ contains at least $2(k-|S|)\cdot d/\rho +1$ vertices combined with the fact that $|O_{i-1}|\leq 2(k-|S|)$ and hence the vertices in $O_{i-1}$ collectively have at most $2(k-|S|-1) \cdot d/\rho$ neighbors in $X_i$.
 
% We demonstrate our proof through the inductive construction of the set OO. We start by setting O0=∅O0​=∅. At the ii-th step, where i∈[k−∣S∣]i∈[k−∣S∣], we select two vertices from XiXi​ that are non-adjacent in HρHρ​ and have no edges connecting them to any vertex in Oi−1Oi−1​. These vertices are then added to Oi−1Oi−1​ to form OiOi​, and ultimately, we define O=Ok−∣S∣O=Ok−∣S∣​. This process is feasible because δ(Hρ)≤dkρδ(Hρ​)≤ρdk​ and XiXi​ contains more than 2(k−∣S∣)dρ+1ρ2(k−∣S∣)d​+1 vertices. Given that ∣Oi−1∣≤2(k−∣S∣)∣Oi−1​∣≤2(k−∣S∣), the vertices in Oi−1Oi−1​ collectively have at most 2(k−∣S∣−1)dρρ2(k−∣S∣−1)d​ neighbors in HH.




\end{proof}



\begin{lemma}
For any $E\subseteq \mathcal{A}$, there are at most $d/\alpha$ elements that are each contained in at least $\alpha\cdot |E|$ many sets from $E$. 
\end{lemma}
\begin{proof}
Assume for contradiction that there are at least  $d/\alpha+1$ such elements denoted by $U'$.  Observe that the total number of sets covered by $U'$ with repetitions is at least $(d/\alpha + 1) \cdot \alpha |E| \ge d|E| + 1$. By the pigeonhole principle, there must exist a set in $E$ containing at least $d + 1$ elements, which leads to a contradiction.
\end{proof}


\subsection{Dominating Set}
\begin{lemma}\label{domset}Let $G=R_0\uplus B_0$ be an instance of a  \textsc{Red Blue Dominating Set} where $|R_0|=r$, $|B_0|=b$, with $r<2b$ and $deg(v)\geq 2$ $\forall v \in B$. There exists $D\subseteq R_0$ of size at most $1/3(b+r)$, such that $N(D)=B_0$.
\end{lemma}
\begin{proof}
We prove the above by constructing a set $D$ with the desired properties. We include a vertex in each round into $D$ and modify the input instance as follows. 

If there is a vertex $r\in R_i$ with at least two neighbors in $B_i$, we include $r$ into $D$. Following this inclusion, we update the instance by deleting $r$ and all its neighbors from the instance, i.e., $R_{i+1}=R_i\setminus\{r\}$, $B_{i+1}=B_i\setminus N(r)$, $G_{i+1}=G[R_{i+1}\uplus B_{i+1}]$. Note that as long as $|R_i|\leq 2|B_i|$, there is always a vertex in $R_i$ with degree at least 2. Suppose the inclusion process ends after $a rounds$. Then, $|R_{a+1}| \geq 2|B_{a+1}|$. Let $F_i$ be any two arbitrary vertices deleted in round $i$ from $B$ and $B'= ((\bigcup_{i=1}^{a} F_i)\cup B_{a+1})\subseteq B$. Now, we extend $D$ to a dominating set of size $1/3(b'+r)$ where $b'=|B'|$. For every vertex $v\in B_{a+1}$, we add one of its neighbor to $D$.
Note that $|B_{a+1}|=b'-2a$ (from construction) and $r-a=|R_{a+1}| \geq 2B_{a+1}$. Putting these two equations together we get, $r-a\geq 2(b'-2a)\implies a\geq 1/3(2b'-r)$.
But, $|D|\leq a + |B_{a+1}| \leq b'-a \leq 1/3(b'+r)$. This consequently bounds the size of $D$ by $1/3(b+r)$.
\end{proof}


% \subsection{$\rho$-independence}
% \todo{define $\rho$-independence definition}
% Given an instance $(U,\mathcal{A},cap)$ of    \textsc{Capacitated $d$-Hitting Set}, we capture the notion of $\rho$-independence among the elements of $U$, with the following defined auxiliary graph $H_{U,\mathcal{A}}$ where $V(H)=U$. Two elements $a$ and $b$ are $\rho$-independent (equivalently adjacent in $H$) if the number of sets in $\mathcal{A}$ containing both $a$ and $b$ are less than $\rho$ fraction of the number of sets containing $a$ as well as less 
% less than $\rho$ fraction of the number of sets containing $b$. Formally, $(a,b)\in E(H)$ if and only if $|(\mathcal{A}\odot a) \cap (\mathcal{A}\odot b)| > \rho \cdot \text{min}\{|(\mathcal{A}\odot a)|, |(\mathcal{A}\odot b)|\}$. 
% We denote $H_{U,\mathcal{A}}$ with $H$, when the context is clear. 

% \begin{lemma}
% $\delta(H) \leq d/\rho$.
% \end{lemma}

% \begin{proof}
%  Let $x\in V(H)$ be a vertex with degree more than $d/\rho$. From the construction of $H$ $\forall y\in N_H(x)$, $|\mathcal{A}\odot y\cap |\mathcal{A}\odot x|> \rho \cdot |\mathcal{A}\odot x|$. Since $\sum_{y\in N_H(x)} |\mathcal{A}\odot y|\cap |\mathcal{A}\odot x|>(d/\rho)\cdot(\rho\cdot |\mathcal{A}\odot x|)= d \cdot |\mathcal{A}\odot x|$, by pigeonhole principle, there exists a set in $|\mathcal{A}\odot x|$ that is present $|A\odot y|$ for $d+1$ many distinct $y$s in $N_H(x)$, a contradiction to the fact that any set has at most $d$ elements. Hence the maximum degree of $H$ is $d/\rho$.   
% \end{proof}

This degree-bound guarantees a $\rho$-independent set (in $H_{U,\mathcal{A}}$) of size $n'$ among any $n'.d/\rho$ elements (vertices in $H_{U,\mathcal{A}}$), which plays a crucial role in the construction of our algorithm. Ideally one would want the elements covering elements of $\mathcal{A}$ to have as less intersection as possible with large $cap$ values. But for our approximation algorithm, we show either there are few elements that are \emph{candidates} for our approximate solution in which case we branch on the choice of an element to be in our solution, or there exists an element that is $\rho$-independent with the other elements of a being constructed solution, which proves to be sufficient in the construction of our approximation algorithm.  




\subsection{Running Time}
Let $R(k')$ denote the running time of {\textsc{CapHS}$(S)$} where $|S|=k-k'$. We prove an upper-bound on $R(k')$ with the following set of recurrence equations resulting from the algorithm.

\begin{align}
R(k')=\underbrace{e^k}_\text{steps 2-3}.\underbrace{2^{k^2}.{(\log_{1+1/k}n)}^{k^2}}_\text{step 7}\{\underbrace{k.n^{\mathcal{O}(1)}}_\text{steps 9-12}+ \underbrace{k.f(k).R(k'-1)}_\text{steps 13-14}+
\underbrace{k^2.n^{\mathcal{O}(1)}}_\text{steps 16-23}
+\underbrace{k^2.f(k).R(k-1)}_\text{step 24}+\underbrace{n^{\mathcal{O}(1)}}_\text{steps 24-29}\}
\end{align}
\todo{are we computing a minimum size dominating set or a \emph{good} dominating set in poly time}
\begin{align}
R(0)=\mathcal{O}(1)
\end{align}

\subsection{(Correctness of) The Algorithm}
\paragraph{Step 0: (Finding $S$):} 
Let $\mathcal{A}_{(S,X)}$, where $X\subseteq S$, denote all the sets in $\mathcal{A}$ whose intersection with $S$ is precisely $X$, i.e., $\mathcal{A}_{(S,X)}=\{A\in\mathcal{A}: A\cap S=X\}$. $\mathcal{A}_{(S,X)}$s are referred to as the \emph{equivalence classes/partitions} of $\mathcal{A}$ with respect to $S$. The following lemma helps us find a desired $S$ that covers \emph{almost} all the sets in $\mathcal{A}_{(S,X)}$, $\forall X \subseteq S$.
\begin{lemma} \label{Sconstruction}
Given an instance $(U,\mathcal{A},cap)$ of \textsc{Capacitated $d$-Hitting Set}, in $g(k,d)n^{\mathcal{O}(1)}$ time, we can find a set $S\supseteq U$ of size at most $k$ such that there is an optimal solution, say $\mathbb{OPT}\supseteq S$, and for every $X\subseteq S$, $S$ covers at least $1 - \frac{1}{f(k)}$ fraction of  $\mathcal{A}_{(S,X)}$.
\end{lemma}

\begin{proof}
For contradiction suppose there exists an $X\subseteq S$ such that $S$ is unable to cover $1 - \frac{1}{f(k)}$ fraction of $\mathcal{A}_{(S,X)}$. We guess $X$, randomly select a set from  $\mathcal{A}_{(S,X)}$, and then branch on its at most $d$ elements that is part of an optimal solution. With a probability of at least $1/2^k\cdot 1/f(k) \cdot 1/d$, we find a vertex $x\in \mathbb{OPT}\setminus S$. We set $S=S\cup\{x\}$, thus increasing the size of $S$.  And $S\subseteq \mathbb{OPT}$ ensures that at most $k$ vertices are included into $S$. Hence the entire construction process of $S$ runs in time $2^k\cdot f(k) \cdot d \cdot n^{\mathcal{O}(1)}$ time.
\end{proof}
\todo{define good S}
% Observe that the sets in $\mathcal{A}$ are categorized based on their neighborhoods in $S$, which limits the number of equivalence classes for the sets in $\mathcal{A}$ to $2^{|S|}$. Furthermore, we uphold the invariant that at least $1 - \frac{1}{f(k)}$ of the sets in each equivalence class are already covered. If this condition is not met, we

% Note that the sets in $\mathcal{A}$ are classified based on their neighborhood in $S$, which bounds the number of equivalence classes for the sets in $\mathcal{A}$ by $2^|S|$. Additionally, we maintain the invariant that from every equivalent class at least $1-1/f(k)$ sets are already covered, otherwise we pick a set randomly from the equivalent class where less than $1-1/f(k)$ fraction sets are covered and branch on one of its elements that belong to an optimal solution, thus increasing the size of $S$ and equivalently discovering another vertex of an optimal solution say $\mathbb{OPT}$.

\paragraph{Steps 2-5: (The Coloring Phase)} Once we obtain a desired $S$, we color the remaining elements of $U\setminus S$ with $r=k-s$ colors. We denote the elements colored with color $i$ by $C_i$. In a \emph{good} coloring, each color class $C_i$ contains an element from $\mathbb{OPT}\setminus S$. And the probability of a coloring being \emph{good} is at least $(1/e^k)$).

\todo{define good coloring $C_i$}
\paragraph{Steps 6-9: (Stars Construction and The Coverage Guessing)} Following a \emph{good} coloring, we guess a partition of the  $2^{|S|}$ many equivalence classes of $\mathcal{A}$ w.r.t $S$ into $S$ parts (each part is known as a \emph{star}). These stars are centered around elements of $S$ and defined by a map $\pi:2^S \rightarrow S$. And a star centered around an element $y\in S$ contains those specific equivalence classes in which $y$ in $\mathbb{OPT}$ covers the maximum number of sets among all the elements of $S$. 
\begin{figure}[H]
\includegraphics[scale=.75]{diagram-20240617.pdf}
\caption{Stars with centers in $S$ and equivalence classes as leaves}
\end{figure}
% Each star has a vertex $y \in S$ as its center, with those equivalence classes as leaves where $y$ covers the maximum number of their sets in the optimal solution $\mathbb{OPT}$. 
Along with guessing $\pi$, for each element in a color class $i \in [r]$ from $\mathbb{OPT} \setminus S$, we estimate its total approximate coverage in all the equivalence classes together centered at $y \in S$, denoted by $\gamma(i, y)$. The sets from $\mathcal{A}$ in a star centered at $y \in S$ are denoted by $\mathcal{A}_y$. Since guessing the exact coverage remains impossible in FPT time (which involves $n^k$ choices), we estimate the approximate coverage, allowing for an error of up to a factor of $1/k$. Specifically, we guess a value $p$ where $0 \leq p \leq t =\log_{1+1/k} |\mathcal{A}|$, such that ${(1+1/k)}^p \leq \gamma(i, y) \leq {(1+1/k)}^{p+1}$. The number of guesses for $\pi$ and the approximate coverage of the $r$ elements of $\mathbb{OPT}$ in $s$ stars are upper bounded by $2^{k^2}$ and  ${(\log_{1+1/k}n)}^{k^2}$, respectively.








%Notice each star has a vertex $y\in S$ as its center with those equivalent classes as leaves that have maximum number of their sets covered by $y$ in $\mathbb{OPT}$. 
% Also for each vertex of a color-class $i\in [r]$ from $\mathbb{OPT}\supseteq S$, we guess its approximate coverage in each equivalence class $y\in S$ denoted by $\gamma(i,y)$.We denote the sets from $\mathcal{A}$ in a star centered at $y \in S$ by $\mathcal{A}_y$. Note that since guessing the exact coverage remains impossible in FPT time ($n^k$ choices), we guess the approximate coverage that is allowed to make an error but only upto an $1/k$ factor, i.e. we guess $p$ where $0\leq p\leq t \log_{1+1/k} |\mathcal{A}|$ and ${(1+1/k)}^p \leq \gamma(i,y)\leq {(1+1/k)}^{p+1}$. 

\paragraph{Steps 10-14: (Filtering  the \emph{candidate elements})} 
For each element in a color class $i$ of $\mathbb{OPT}$, we denote its total approximate coverage across all stars in $\mathbb{OPT}$ by $\delta_i$. From a color class, we only select those elements into the set $C_i'$ that are capable of making such a coverage contribution. This is done by checking if an element $x\in C_i$ has the required capacity, i.e., $cap(x) \geq \delta_i$, and if it can cover the required number of sets in each star, i.e., $|\mathcal{A}_y \odot x| \geq \gamma(i, y)$ for all $y \in S$. Any element satisfying both these requirements is known as a \emph{candidate} element and is selected into $C_i$'. Additionally, if any of the sets $C_i'$ contains fewer than $f(k)$ vertices, we can branch and find another vertex of $\mathbb{OPT}$, and include it into $S$. Following which we repeat the construction procedure described in Lemma \ref{Sconstruction} to get a desired $S$ of strictly larger size.
\textcolor{red}{Henceforth, we may assume that each $C_i$' contains at least $k$ candidate elements.}

%For each vertex in the color class i of $\mathbb{OPT}$, we denote its total approximate coverage in $\mathbb{OPT}$ (to all the stars) by $\delta_i$. And from a color class we filter out all the candidate vertices into $C_i'$ capable of making such a coverage contribution by checking if the vertex $x$ has the required capacity $cap(x)\geq \delta_i$ and if it can hit the required no of sets in each star by checking  $|\mathcal{A}_y \odot x| \geq \gamma(i,y) \text{ for all } y \in S$. If any of the sets $C_i'$ contains less than $f(k)$ vertices we can branch and find another vertex of $\mathbb{OPT}$.

\paragraph{Steps 15-23: (Finding the best candidates and \emph{star-dominating} color classes)} For each star $y$, we guess the color of the vertices in $\mathbb{OPT}$ that makes the highest and second highest contribution (say $j$) (break ties arbitrarily) denoted by $i_y$ and $j_y$, respectively ($i_y$ and $j_y$ color classes \emph{star-dominate} $y$). Additionally, for each vertex in $U\setminus S$, we track its capacity to cover additional sets in each star $y$ with a value $scr_y(x)$. The higher the $scr_y(x)$ value, the more the element $x$ can cover additional sets in star $y$ after fulfilling its required quota of sets to cover in other stars. Thus, $scr_y(x)$ is defined as the minimum between the number of sets $x$ is contained in within $A_y$ and the number of sets it can cover in $A_y$ after meeting its required quota of sets to cover in other stars. Formally, $\mathsf{scr}_y(x) \leftarrow \min\{|\mathcal{A}_y \odot x|,\mathsf{cap}(x)-\delta_i+\gamma(i,y)\}$. From each $C_i'$, for each star $y$, top $f(k)$ elements with highest $scr_y$ are selected into $C_i''$. Note that barring for the intersection of sets covered by elements, these sets ($C_i''$) contain the best \emph{candidates} to cover sets in each star. Next we branch on the possibility if $\mathbb{OPT}$ contains an element from one of the $C_i''$s or not. If it does, we guess the element and include it into $S$. Following which we repeat the construction procedure
described in Lemma \ref{Sconstruction} to get a desired $S$ of strictly larger size. Otherwise, we do the following.

% Additionally, with each vertex in $U\setminus S$, we keep track of its ability to cover additional sets in a each star $y$ with a value $scr_y(x)$. The higher the $scr_y(x)$ value is the more the element $x$ can cover additional sets in the star $y$ after covering the necessary amount of sets in other stars. Hence $scr_y(x)$ is defined to be the minimum value between the number of sets $x$ is contained in $A_y$ and the number of sets it can hit in $A_y$ after fulfilling its reuiqremtn quoata of sets to hit in other stars, i.e., formally $\mathsf{scr}_y(x) \leftarrow \min\{|\mathcal{A}_y \odot x|,\mathsf{cap}(x)-\delta_i+\gamma(i,y)\}$  and in \todo{some confusion about score function} 

\paragraph{Steps 25:29}

We call a color class \emph{heavy} if it is the highest contributing color class to at least two different stars, else we call it a \emph{light} color class. The heavy colorclasses are denoted by $X$. We begin with the following observation, which represents the final step in the design of our approximation algorithm. This observation states that selecting an additional element each from a \emph{star-dominating} color classes which includes $X$,
along with one element from each color class in $[r]$, that together forms a $\rho$-independent set, compensates for the loss of sets resulting from the $1/k$ factor loss while guessing the approximate coverage (and choosing an arbitrary candidate vertex that is part of some $\rho$-independent set) and the at most $\rho$ fraction of sets that might be common among a pair of the already chosen elements.
% \todo{may be define star dominating set instead of star dominating color classes}
The following lemma holds based on the fact no $C_i''$ contains an element from $\mathbb{OPT}$.
\begin{lemma}Let
$G \leftarrow \textsc{Bipartite}([r],S,\{(i_y,y): y \in S\} \cup \{(j_y,y): y \in S\})$ and $X \leftarrow \{i \in [r]: |\{y \in S: i_y = i\}| \geq 2\}$. Let $D\subseteq[r]$ satisfying $X\subseteq D$ and $N_G(D)=S$ and
$R \subseteq \bigcup_{i=1}^r C_i''$ satisfying that 

\ \ \ \ \ \ \ \ \ \ $\bullet$ $|R \cap C_i''| = 2$ for $i \in D$
                
                \ \ \ \ \ \ \ \ \ \ $\bullet$ $|R \cap C_i''| = 1$ for $i \in [r] \backslash D$

                \ \ \ \ \ \ \ \ \ \ $\bullet$ $R$ is $\frac{1}{k^2}$-almost $\mathcal{A}_y$-independent for all $y \in S$.
                \ \  \  \  \  \ \ \ \

\noindent Then $S\cup R$ is a feasible solution if no $C_i''$ contains an element from $\mathbb{OPT}$. 
\end{lemma}

                
                
% We claim that $S\cup R$ is a feasible solution. Let $D\subseteq R$ be a computed dominating set on the bipartite graph $G$ defined in line 25.
% \begin{proof}
% Note that $R$ includes one vertex from each color class (outside $D$) and exactly two vertices from the color classes in $D$. We assert that $R$ is $1/k^2$-independent in the auxiliary (degenerate) graph since the number of elements in each $C''_i$ is exactly $f(k)$. \textcolor{red}{ replace eqv classes by stars and the arguments still hold} Let $s'$ denote the size of an equivalence class (denoted Eq) covered by vertices from the color classes $r' \subseteq r$, with $i$  and $j$ being the respective color classes covering the highest and second highest number of sets from the equivalence class. The sum of the coverage by $R \setminus D$ for the equivalence class $Eq$ is at least $s' \cdot (1 - 1/k)$ (From Step 7). However, this does not necessarily represent the number of sets from the equivalence class that may be covered by $R$, as there may be elements $x, y \in R$ such that $Eq \odot x \cap Eq \odot y \neq \emptyset$. However, since the elements in $R$ are independent (in the degenerate graph), the maximum number of sets that are hit by more than one element from $R \setminus D$ is bounded above by $\sum_{x, y \in R \setminus D} |Eq \odot x \cap Eq \odot y| \leq \sum (1/k^2 \min\{|Eq \odot x|, |Eq \odot y|\} n) \leq \binom{k}{2} \cdot (1/k^2) \cdot j_{Eq}$.
% (here jEq denoted the coverage of the second highest element in the star/eqv class Eq)

%  \textcolor{red}{take $1/k^3$ independent set and you can cover upto k stars that are dominated by a single additional vertex}
%  An additional vertex from dominating set covering $j_{Eq}$ sets will cover at least $(1-1/k)j_{Eq}$ additional sets in $Eq $ that are not covered by $R\setminus D$, thus making up for the at most 1/2k sets that are overcounted (counted at least twice).
% Hence $S\cup R$ is a feasible solution as the same argument can be made for any equivalent class.\end{proof}

\begin{proof}
Note that $R$ includes one vertex from each color class (outside $D$) and exactly two vertices from the color classes in $D$. We assert that $R$ is $1/k^2$-independent (\textcolor{red}{may be explain why such a set always exists with degree bound argument?}) in the auxiliary (degenerate) graph since the number of elements in each $C''_i$ is exactly $f(k)$. Let $R_1\subseteq$ be a set of $r$ elements each from a unique color class. 

We argue that all the sets in a star $A_y$ are covered by $S\cup R$ with the following two exhaustive cases.

\begin{itemize}
    \item Case 1: ($A_y$ is dominated by a colorclass in $X$, say $H$)- Let $s'$ denote the number of sets in $A_y$ covered by elements in $\mathbb{OPT}\setminus S$. In this case there are at least 2 vertices $a,b$ selected from $H$ into $R$. W.l.g $a\notin R_1$. Note that the sum of coverage by the elements in $ R_1 $ for $A_y$ is at least $s' \cdot (1 - 1/2k)$ \textcolor{red}{(we make it 2k in the approximating coverage part)} (From Step 7). However, this does not necessarily imply that the number of sets from $A_y$ that may be covered by $ R_1$, as there may be elements $x, y \in R_1$ such that $(A_y \odot x) \cap (A_y \odot y) \neq \emptyset$.  But, since the elements in $R$ (including a) are $\rho$-independent (in the degenerate graph), the maximum number of sets that contain more than one element from $ R_1\cup \{a\}$ is upper-bounded by $\sum_{x, y \in R_1\cup\{a\}} |A_y \odot x \cap A_y \odot y| \leq \sum_{x, y \in R_1\cup\{a\}} \rho \cdot \min\{|A_y \odot x|, |A_y \odot y|\} n) \leq \binom{k+1}{2} \cdot \rho \cdot j_{A_y}$ (here $j_{A_y}$ denotes the coverage of the second highest element in  $S_y$). If we choose $\rho=1/k^3$, the number of sets that may be double counted is at most $1/2k\cdot s'$. Including $a$ ($a$ being independent with rest of the elements in $R_1$), we cover at least $scr_y(a)\geq s'/k$ new sets which is at least as much as the number of sets lost while guessing approximate coverage ($s'/2k$), and with double counting sets($s'/2k$). \textcolor{blue}{Redistribution routine using center $y$}
     \item Case 2: ($A_y$ is dominated by a colorclass outside $X$, say $H$)
     In this case let $z$ be the color class that contributes the maximum to $A_y$. Note that $z$ does not contribute maximum to any other stars otherwise $z\in X$. Now while choosing a vertex from $z$ (in $R_1$), we choose a vertex from Top($C'_z,scr_y,f(k)$). Note that any such vertex can cover at least as many sets in $A_y$  than $\mathbb{OPT}\cap C_z$ because of its higher(greater or equal to) $scr_y$ value. Hence we avoid losing sets $1/2k$ fraction of sets while guessing approximate coverage. Let $s'$ denote the number of sets in $A_y$ covered by elements in $\mathbb{OPT}\setminus S$ and $b$ be a vertex that we choose from $C_H$. Then the number of sets we lose is only because of double counting of sets which again is upper bounded by $\binom{k+1}{2} \cdot \rho \cdot j_{A_y}$. If we choose $\rho=1/k^3$, the number of sets that may be double counting is at most $1/2k\cdot j_{A_y} $ which is easily compensated by the $j_{A_y}$ additional number of sets covered by $b$. \textcolor{blue}{Redistribution routine using center $y$}

     \item Redistribution routine using center $y$: Note that $y$ being the vertex that covers the maximum in each equivalence class of star $S_y$ covers at least $1/k\cdot (1-1/f(k))$ fraction from each equivalence class present in $S_y$.The number of  sets that remain uncovered $s'$ in each equivalence class is at most $1/f(k)$. Additionally all sets in star contain the element $y$. 
     
     %And all the additional sets that are covered by the additional dominating element $a$ (at least $(1-1/k)\cdot j_{A-y}$ many) were originally covered by $y$ in $\mathbb{OPT}$. This we can ensure because of the following fact. 

    Let $E_1,...,E_i$ be the $i$ equivalence classes where
   the number of sets that can not be covered by $S\cup R_1$ is $z_1,...,z_i$. Let $a$ cover $x_1,...,x_i$ many sets in each equivalence class that are that do not contain any elements from $R$ other than $a$. And $\sum_i{z_i}\leq \sum_i{x_i}$ (by properly selecting $\rho$ and the log factor). Also each $z_i$ is less than the number of sets $y$ covers in $E_i$ (be careful here with arguments). We could have redistribute the sets covered in $E_i$ among the elements of $S$ in $\mathbb{OPT}$ such that $y$ would cover at least $z_i$ many sets. But these $z_i$ (in fact $x_i$) many sets now being covered by $a$ ensures that at least $z_i$ amount of coverage of $y$ in $E_i$ is freed up. Together from all the equivalence classes  $\sum_i{z_i}$ amount of coverage from $y$ is freed which it can now use to cover $z_i$ many sets that were intially not covered by $S\cup R_1$. The same arguments can be repated on any stars to make sure that $S\cup R$ covers all the sets in every star thus making it a feasible solution.    
\end{itemize}









% Let $s'$ denote the number of sets in a star $A_y$ whose sets are covered by elements from the color classes $r' \subseteq r$ in $\mathbb{OPT}$, with $i$  and $j$ being the respective color classes covering the highest and second highest number of sets from $A_y$. Note that the sum of coverage by the elements in $R \setminus D$ for $A_y$ is at least $s' \cdot (1 - 1/k)$ (From Step 7). However, this does not necessarily imply that the number of sets from $A_y$ that may be covered by $R\setminus D$, as there may be elements $x, y \in R \setminus D$ such that $(A_y \odot x) \cap (A_y \odot y) \neq \emptyset$.  However, since the elements in $R$ are $\rho$-independent (in the degenerate graph), the maximum number of sets that contain more than one element from $R \setminus D$ is upper-bounded by $\sum_{x, y \in R \setminus D} |A_y \odot x \cap A_y \odot y| \leq \sum \rho \cdot \min\{|A_y \odot x|, |A_y \odot y|\} n) \leq \binom{k}{2} \cdot \rho \cdot j_{A_y}$ (here $j_{A_y}$ denotes the coverage of the second highest element in  $S_y$). If we choose $\rho=1/k^3$, at most $j_{A_y}$ many sets contain more than one elements then an additional vertex dominating a star $y$ can cover an additional $j_{A_y}$ sets 

\end{proof}


\subsection{Approximation ratio}
We show that our algorithm returns a solution ($S\cup O$) of size at most $\frac{4k}{3}$ by considering the following two exhaustive cases.
\begin{itemize}
    \item \textbf{Case 1 ($k-|S|<2|S|$)}: In this case we show the existence of a dominating set $D'$ such that such that $|D'\cap X''_i|\geq 2$ for each $i\in [k-|S|]$ such that $|\tau^{-1}(i)|\geq 1$. For each $i\in [k-|S|]$ such that $|\tau^{-1}(i)|\geq 1$ (say $x$ many), we include $i$ into $D$ and delete the vertices in $S$ that are already dominated. With the inclusion of every such $i$ size of $H$ decreases by (1 since $i$ is included and at least 2 vertices of $S$ dominated by $i$ in $H$). After an exhaustive application of such an inclusion procedure $|V(H)\leq s-2x+k-x=k-3x|$. And Lemma \ref{domset} implies an existence of a dominating set $D'$ of size at most $x+1/3(k-3x)=\frac{k}{3}$. Therefore, we have the following upper bound on the size of the found solution: $|S\cup O|=|S| + k-s + |D| \leq |S| + k-s + |D'| \leq k + s \leq \frac{4k}{3}$.
    
    \item \textbf{Case 2 ($k-s\geq 2s$)}:
    In this case, there is a set $D'\in[k-s]$ dominating $S$ in $H$  where $D'=\{\tau_1(s)|s\in S\}$ such that $|D'\cap X''_i|\geq 1$ for each $i\in [k-|S|]$ such that $|\tau^{-1}(i)|\geq 2$. Therefore, we have the following upper bound on the size of the found solution: $|S\cup O|=|S| + k-s + |D| \leq |S| + k-s + |D'| \leq k + s \leq \frac{4k}{3}$ (since $k-s\geq 2s\implies s\leq k/3$).
\end{itemize}


\textcolor{red}{tree argument not required}

==> abstract.tex <==
In the \textsc{Capacitated $d$-Hitting Set} problem input is a universe $U$ equipped with a capacity function $\mathsf{cap}: U \rightarrow \mathbb{N}$, and a collection $\mathcal{A}$ of subsets of $U$, each of size at most $d$. The task is to find a minimum size subset $S$ of $U$ and an assignment $\phi :  \mathcal{A} \rightarrow S$ such that, for every set $A \in \mathcal{A}$ we have $\phi(A) \in A$ and for every $x \in U$ we have $|\phi^{-1}(x)| \leq \mathsf{cap}(x)$. Here $\phi^{-1}(x)$ is the collection of sets in $\mathcal{A}$ mapped to $x$ by $\phi$. Such a set $S$ is called a {\em capacitated hitting set}. When $d=2$ the problem is known under the name  \textsc{Capacitated Vertex Cover}. In  \textsc{Weighted Capacitated $d$-Hitting Set} each element of $U$ has a positive integer weight and the goal is to find a capacitated hitting set of minimum weight. 

Approximation algorithms for \textsc{Capacitated Vertex Cover} were first studied by Chuzhoy and Naor [SICOMP 2006], who gave a factor $3$ approximation algorithm for \textsc{Capacitated Vertex Cover} and showed that the weighted version does not admit an $o(\log n)$-approximation unless P=NP. 
 %
After a series of improvements spanning a period of 15 years, Kao [SODA 2017] and Wong [SODA 2017] independently obtained $d$-approximation algorithms for \textsc{Capacitated $d$-Hitting Set}.
%
This matches the ratio for the classic \textsc{$d$-Hitting Set} problem, and therefore cannot be improved to $d-\epsilon$ for any $\epsilon > 0$ assuming the Unique Games Conjecture. 
%
\textsc{Capacitated Vertex Cover} is also well understood from the perspective of parameterized algorithms: van Rooij and van Rooij [SOFSEM 2019] gave a $k^k|U|^{O(1)}$ time algorithm to determine whether there exists a solution $S$ of size at most $k$, showing that the unweighted problem is {\em fixed parameter tractable} (FPT) parameterized by the solution size $k$.

In this paper we initiate the study of parameterized (approximation) algorithms for \textsc{Capacitated $d$-Hitting Set}. An easy reduction shows that, as opposed to \textsc{Capacitated Vertex Cover}, unweighted \textsc{Capacitated $d$-Hitting Set} for $d \geq 3$ does {\em not} admit an FPT algorithm unless FPT=W[1]. 
%
Our main result is a parameterized approximation algorithm that runs in time 
$\left(\frac{k }{\epsilon} \right)^k 2^{k^{\cO(kd)}}(|U|+|\mathcal{A}|)^{O(1)}$ 
and either concludes that there is no solution of size at most $k$ or outputs a solution $S$ of size at most $4/3 \cdot k$ and weight at most $2+\epsilon$ times the minimum weight of a solution whose size is at most $k$.
%
We note that while the running time of our algorithm depends on $d$, the approximation ratio does not. 
%
Thus this parameterized approximation algorithm achieves a ratio smaller than what can be achieved by polynomial time approximation algorithms with a running time that is faster than what can be achieved by an algorithm solving the problem exactly. 
%
%
We complement our algorithmic results by showing that there exists a constant $c > 1$ such that for every $d \geq 3$, assuming the Exponential Time Hypothesis, there is no FPT-approximation algorithm for unweighted \textsc{Capacitated $d$-Hitting Set} with approximation factor $c$, and no factor $2-\epsilon$ FPT-approximation algorithm for weighted \textsc{Capacitated $d$-Hitting Set}. These hardness results even hold for \textsc{Capacitated Vertex Cover} in multigraphs. On the way we show that a variant of multi-dimensional {\sc Knapsack} is hard to FPT-approximate within a factor $2-\epsilon$. This result may be of independent interest. 


==> algorithm_old.tex <==
\section{Main Algorithm}

\textbf{Technical Overview:}
\begin{itemize} 
    \item Talk about equivalence class and its flexibility since each has same neighborhood
    \item 90\% coverage by $S$
    \item Two from each color class with independence notion
    \item Talk about stars and their use to improve approximation factor
    \item Now talk about top and second top to obtain similar guarantees for notS in every star
\end{itemize}
%First we reduce \textsc{Capacitated $d$-Hitting Set} to a new auxiliary problem that we define below.
%


Given a set $S$, let $\mathcal{P}(S)$ denote the family of all subsets of $S$. Our algorithm at any point has a partially constructed solution $S$. We make some guesses to include an additional vertex to $S$ and solve the problem recursively. We first define a notion that captures the form of the guesses we make and thus the subproblems we solve. Suppose $S$ is a partial solution, then we store information with respect to each $E\in \cP(S)$. Let $A_E$ be the sets $A \in \cA$ such that $A\cap S=E$. We store (i) an estimate of how much each vertex in the solution covers in $A_E$ and (ii) the element of $S$ that contributes the maximum to $A_E$. We also store a partition of $U\setminus S$ such that each part contains at most one solution vertex. We formalize the required notions and the subproblem we solve below.

\todo{figure for annotated tuple and good annotated tuple}
\begin{definition}
    An annotated tuple is a tuple $(S,X=X_1\uplus \cdots \uplus X_{k-|S|},\pi,\gamma)$ where
    \begin{itemize}
        \item $S,X\subseteq U$ with $|S|\leq k$ and $X\cap S=\emptyset$
        \item $\pi: \mathcal{P}(S)\rightarrow S$
        \item $\gamma: ([k-|S|] \cup S) \times \mathcal{P}(S) \rightarrow \{\lceil (1+\frac{1}{k})^p \rceil: p \in [|\cA|]\}$
    \end{itemize}
    We extend $\gamma$ to the domain $([k-|S|]\cup S) \times S$ by defining for each $i\in [k-|S|]\cup S$ and $s\in S$, $$\gamma(i,s):=\sum_{E\in \pi^{-1}(s)}\gamma(i,E)$$
    %E\in \cP(S):\pi(E)=s
    %
    For each $E\in \cP(S)$ and $s\in S$, we define 
    $$\cA_E:=\{A\in \cA: A\cap S=E\}$$
    $$\cA_s:=\{A\in A_E: \pi(E)=s, E\in \cP(S)\}$$
    %
    When $S=\emptyset$, $\cP(S)=\emptyset$ and so $\pi$ and $\gamma$ have an empty domain or co-domain. We denote the annotated tuple in this case by $(\emptyset,X,.,.)$
\end{definition}

\begin{definition}
    An annotated tuple $(S,X,\pi,\gamma)$ is good if there exists a solution $S^*$ to $\capinstance$ along with an assignment $\phi^*:\mathcal{A}\rightarrow S^*$ such that
    \begin{enumerate}
        \item $S\subseteq S^*$
        \item For each $X_i$, $i\in [k-|S|]$, $|X_i\cap S^*|=1$
        \item For each $s\in S$ and $E\in \mathcal{P}(S)$, $\gamma(s,E)=\lfloor \log_{1+\frac{1}{k}} |\phi^{-1}(s)\cap \cA_E| \rfloor$
        \item For each $i\in [k-|S|]$ and $E\in \mathcal{P}(S)$, $\gamma(i,E)=\lfloor \log_{1+\frac{1}{k}} |\phi^{-1}(S^*\cap X_i)\cap \cA_E| \rfloor$
        \item For each $E\in \mathcal{P}(S)\setminus \emptyset$, $\pi(E)=\max_{s\in S}|\phi^{-1}(s)\cap \cA_E|$
    \end{enumerate}
    We also say $(S,X,\pi,\gamma)$ is good due to solution $S^*$.
\end{definition}

\begin{observation}
\label{observation:empty-good-tuple}
$(\emptyset,X,.,.)$ is good if there exists a solution $S^*$ with $|X_i\cap S^*|=1$ for each $i\in [k]$.
\end{observation}

\begin{lemma}
\label{lemma:annotated-d-hs}
    There exists an algorithm that takes as input an instance $\capinstance$, an annotated tuple $(S,X,\pi,\gamma)$ and in time $f(k)poly(n)$ either returns NO or a solution to $\capinstance$. Further, if $(S,X,\pi,\gamma)$ is good due to a solution $S^*$, $|S^*|\leq k$, it returns a solution of size at most $\frac{4}{3}|S^*|$.
\end{lemma}

\begin{theorem}
\label{theorem:main-alg}
    There exists an algorithm to \capdhs\ that takes as input an instance $\capinstance$ and in time $f(k)poly(n)$ either returns a solution of size at most $\frac{4}{3}k$ or determines there exists no solution of size at most $k$.
\end{theorem}

\begin{proof}
The algorithm does the following:
\begin{itemize}
    \item Construct a hash family $\mathcal{F}$ of set of sets $\{X_1,\cdots,X_k\}$.\todo{hash family}
    \item For each $\{X_1,\cdots,X_k\}\in \mathcal{F}$, use Lemma~\ref{lemma:annotated-d-hs} with $(\emptyset,X=X_1\uplus \cdots \uplus X_k,.,.)$. If the algorithm returns a set of size $S'$ at most $\frac{4}{3}k$, then return $S'$.  
    \item Return NO if no set $S'$ was returned in the previous step.
\end{itemize}

Assume there exists a solution $S^*$ to $\capinstance$ of size at most $k$. Then by construction of $\mathcal{F}$, we know that there exists a $\{X_1,\cdots,X_k\}\in \mathcal{F}$ such that $X_i\cap S^*$ for each $i\in k$. By Observation~\ref{observation:empty-good-tuple}, we know that $(S,X,.,.)$ is good due to $S^*$. Thus invoking Lemma~\ref{lemma:annotated-d-hs} on $(S,X,.,.)$ returns a solution $S'$ to $\capinstance$ of size at most $\frac{4}{3}k$.
%
The time required to construct $\mathcal{F}$ is $ $\todo{}. Each call to Lemma~\ref{lemma:annotated-d-hs} runs in time $ $ and the Lemma is invoked $|\mathcal{F}|$ many times, thus the total runtime is $ $\todo.
\end{proof}

\subsection{Proof of Lemma~\ref{lemma:annotated-d-hs}}

\begin{definition}
   Given sets $S,X\subseteq U$ with $X\cap S=\emptyset$, let $\mathcal{F}_{S,X}$ denote the set of all possible annotated tuples $(S,X,\pi,\gamma)$.  
\end{definition}
We first state our algorithm below:
\begin{itemize}
    \item \textbf{Input:} An annotated tuple $(S,X,\pi,\gamma)$ and $\capinstance$
    \item \textbf{Output: } $NO$ or a solution to $\capinstance$ of size at most $\frac{4}{3}k$
    \item If $|S|=k$ and $S$ is a solution, return $S$ else return $NO$.
    \item For each $i\in [k-|S|]$ define
    $$X_i' \leftarrow \{x \in X_i: \mathsf{cap}(x) \geq \sum_{s \in S} \gamma(i,s) \text{ and } |\mathcal{A}_s \odot x| \geq \gamma(i,s) \text{ for all } s \in S\}$$
    \item For each pair of distinct functions $\tau_1: S\rightarrow [k-|S|]$ and $\tau_2:S\rightarrow [k-|S|]$ do: \todo{Just taking top and secondtop of $\gamma$ should be ok}
    \begin{itemize}
        \item For $i\in [k-|S|]$, $v\in X_i$ and $s\in S$ define $$\score(v,s):=\min\{|\cA_s \odot v|,\capa(v)-\sum_{s'\in S, s'\neq s} \gamma(i,s)\}$$
        \item For each $i\in [k-|S|]$, let $T(i,s)$ be the top $f(k)$ vertices of $X_{i}$ when sorted in non-increasing order of $\score(v,s)$.
        \item For each $i\in [k-|S|]$, construct $X''_i\subseteq X_i$ as $X''_i:=\bigcup_{s\in \tau_{1}^{-1}(i)}T(i,s)$.
        \item For each $i\in [k-1]$ and for each $v\in X''_i$
        \begin{itemize}
            \item Let $S':=S\cup \{v\}$ and $X':=X\setminus X_i$
            \item For each annotated tuple $(S',X',\pi',\gamma')\in \cF_{S',X'}$, apply Lemma~\ref{lemma:annotated-d-hs} on $(S',X',\pi',\gamma')$. If Lemma~\ref{lemma:annotated-d-hs}  returns a set of size at most $\frac{4}{3}k$ return it.
        \end{itemize}
    \item Construct the bipartite graph $H:=(S\uplus [k-s],E)$ where $E:=E_1\cup E_2$, $E_1:=\{(s,\tau_1(s)):s\in S\}$ and $E_2:=\{(s,\tau_2(s)):s\in S\}$.
    \item Find a set $D\subseteq [k-s]$ that dominates $S$ in $H$ such that $\{i\in [k-|S|]:|\tau^{-1}(i)|\geq 2\} \subseteq D$. 
    \item Construct a set $O$ using Lemma~\ref{lemma:conflict-independent-set} such that:
    \begin{enumerate}
        \item $|O\cap X''_i|\geq 1$ for each $i\in [k-|S|]$
        \item $|O\cap X''_i|\geq 2$ for each $i\in D$
        %\item $|O\cap X''_i|\geq 2$ for each $i\in [k-|S|]$ such that $|\tau^{-1}(i)|\geq 2$.
        \item $O$ is $\frac{1}{k^2}$-conflict independent\todo{need stronger for bounds}
    \end{enumerate}
    \item Return $O\cup S$ if it is a solution of size at most $\frac{4}{3}k$
    \end{itemize}
\end{itemize}

It is clear that if the algorithm returns a set it is a solution of size at most $\frac{4}{3}k$. We now need to show that if $(S,X,\pi,\gamma)$ is good due to  a solution of size at most $k$, then the algorithm returns a solution of size at most $\frac{4}{3}k$.

From now, we fix $S^*$ be a solution of size at most $k$ due to which $(S,X,\pi,\gamma)$ is good. We prove that the algorithm returns a solution of size at most $\frac{4}{3}k$ by induction on the size of $S$. Base Case $|S|=k$: In this case  $S\subseteq S^*$ since $S^*$ is a solution due to which $(S,X,\pi,\gamma)$ is good. Further since $|S^*|\leq k$, $S^*=S$ and thus the algorithm returns $S$.

We now assume that the algorithm returns a solution of size at most $\frac{4}{3}k$ for all $S$ of size greater than $\ell$. We prove the claim for $|S|=\ell$. Let $X'':=\bigcup_{i\in [k-s]}X''_i$. We divide our proof into two cases: $(i)$ $S^*\cap X''\neq \emptyset$ and $(ii)$ $S^*\cap X''=\emptyset$.

We first prove case $(i)$. Let $v\in S^*\cap X''$ and $v\in X''_i$. We define $S':=S^*\cup\{v\}$ and $X':=X\setminus X_i$. Since $(S,X,\pi,\gamma)$ is good due to $S^*$, there exists an annotated tuple $(S',X',\pi',\gamma')$ that is good with respect to $S^*$. The algorithm goes over every annotated tuple in $\cF_{S',X'}$ and thus calls Lemma~\ref{lemma:annotated-d-hs} on $(S',X',\pi',\gamma')$. By induction since $|S'|>|S|$, this recursive call returns a solution of size at most $\frac{4}{3}k$.

To complete our proof, we need to prove the claim for case $(ii)$. For this, we first show that $S\cup O$ is a solution.
\begin{lemma}
If $S^*\cap X''=\emptyset$, then $S\cup O$ is a solution to $\capinstance$.


\end{lemma}
\begin{proof}
Let $\phi^*:\mathcal{A}\rightarrow S^*$ be an assignment of $\mathcal{A}$ to $S^*$. We first prove the following claim. 
\begin{lemma}
    If $S^*\cap X''=\emptyset$ then for each $E\in \cP(S)$, 
\end{lemma}
\end{proof}

\begin{lemma}
$|S\cup O|\leq \frac{4}{3}$    
\end{lemma}
\begin{proof} Let $s=|S|$, we divide the analysis into two cases: (i) $k-s<2s$ and (ii) $k-s\geq 2s$. First observe that $|S \cup O|=|S|+k-|S|+|D|=k+|D|$.
For case (i) we use that $|D|\leq \frac{1}{3}(|S|+k-|S|)$ by Lemma~\ref{}. Here $|S\cup O|\leq k+|D|\leq k+1/3(|S|+k-|S|)\leq 4k/3$.
.
    \item \textbf{Case 2 ($r\geq 2s$)}:
    In this case, we can find a dominating set of size $s$. Therefore, we have the following upper bound on the size of the found solution: $|S| + r + |D| \leq k + s \leq \frac{4k}{3}$.
\end{proof}

% \begin{lemma}Let $G=R\uplus B$ be an instance of \textsc{Red Blue Dominating Set} with $|R|=r$ and $|B|=b$ satisfying $r<2b$ and $deg(v)\geq 2$, $\forall v \in B$. Then there exists a red-blue dominating set $D\subseteq R$ of size at most $\frac{1}{3}(b+r)$ that can be found in polynomial time.
% \end{lemma}


% \begin{definition}
%     Let $(S,X,\pi,\gamma)$ be a good tuple due to a solution $S^*$, then a pair of functions $(\tau_1,\tau_2)$ where $\tau_1:S\rightarrow [k-|S|]$ and $\tau_2:S\rightarrow [k-|S|]$ is good if:
%     \begin{itemize}
%         \item For each $s\in S$, 
%     \end{itemize}
% \end{definition}


\subsection{Conflict Independence}
We use the notion of conflict independence crucially in our result.

\begin{definition}
Two element $a,b\in U$ are said to be conflict independent if $a$    
\end{definition}

\begin{lemma}
\label{lemma:conflict-independent-set}
    Given a set $X\subseteq U$, $X=X_1\uplus \cdots \uplus X_{\ell\leq k}$ with $|X_i|\geq $, one can in polynomial time find sets $Y_1,\cdots,Y_\ell$ such that $Y_i\subseteq X_i$, $Y_i\geq 2$ and $\cup_{i\in [\ell]}Y_i$ is $\frac{1}{k^2}$-independent.
\end{lemma}

\section{Conclusion}
Also works for partial $d$-HS with same ratio by the $d$ to $d+1$ reduction.

==> algorithm_old_2.tex <==
\section{Main Algorithm}

\textbf{Technical Overview:}
\begin{itemize} 
    \item Talk about equivalence class and its flexibility since each has same neighborhood
    \item 90\% coverage by $S$
    \item Two from each color class with independence notion
    \item Talk about stars and their use to improve approximation factor
    \item Now talk about top and second top to obtain similar guarantees for notS in every star
\end{itemize}
%First we reduce \textsc{Capacitated $d$-Hitting Set} to a new auxiliary problem that we define below.
%


Given a set $S$, let $\mathcal{P}(S)$ denote the family of all non-empty subsets of $S$. Our algorithm at any point has a partially constructed solution $S$. We make some guesses to include an additional vertex to $S$ and solve the problem recursively. We first define a notion that captures the form of the guesses we make and thus the subproblems we solve. Suppose $S$ is a partial solution, then we store information with respect to each $E\in \cP(S)$. Let $A_E$ be the sets $A \in \cA$ such that $A\cap S=E$. We store (i) an estimate of how much each vertex in the solution covers in $A_E$ and (ii) the element of $S$ that contributes the maximum to $A_E$. We also store a partition of $U\setminus S$ such that each part contains at most one solution vertex. We formalize the required notions and the subproblem we solve below.

\todo{figure for annotated tuple and good annotated tuple}
\begin{definition}
    An annotated tuple is a tuple $(S,X=X_1\uplus \cdots \uplus X_{k-|S|},\pi,\gamma)$ where
    \begin{enumerate}
        \item[(1)] $S,X\subseteq U$ with $|S|\leq k$ and $X\cap S=\emptyset$
        \item[(2)] $\pi: \mathcal{P}(S)\rightarrow S$
        \item[(3)] $\gamma: ([k-|S|] \cup S) \times \mathcal{P}(S) \rightarrow \{\lceil (1+\frac{1}{k})^p \rceil: p \in [|\cA|]\}$
    \end{enumerate}
    We extend $\gamma$ to the domain $([k-|S|]\cup S) \times S$ by defining for each $i\in [k-|S|]\cup S$ and $s\in S$, $$\gamma(i,s):=\sum_{E\in \pi^{-1}(s)}\gamma(i,E)$$
    %E\in \cP(S):\pi(E)=s
    %
    For each $E\in \cP(S)$ and $s\in S$, we define 
    $$\cA_E:=\{A\in \cA: A\cap S=E\}$$
    $$\cA_s:=\{A\in A_E: \pi(E)=s, E\in \cP(S)\}$$
    %
    Given $S$ and $X$ satisfying (1), let $\cF_{S,X}$ denote the set of all possible annotated tuples $(S,X,\pi,\gamma)$

    %
    %When $S=\emptyset$, $\cP(S)=\emptyset$ and so $\pi$ and $\gamma$ have an empty domain or co-domain. We denote the annotated tuple in this case by $(\emptyset,X,.,.)$
\end{definition}

\begin{definition}
\label{definition:good-tuple}
    An annotated tuple $(S,X,\pi,\gamma)$ is good if there exists a solution $S^*$ to $\capinstance$ along with an assignment $\phi^*:\mathcal{A}\rightarrow S^*$ such that
    \begin{enumerate}
        \item $S\subseteq S^*$
        \item $S\cap A\neq \emptyset$ for each $A\in \cA$
        %\item For each $E\in \cP(S)$, $\cov_{\phi^*}(S,E)\geq (1-\frac{1}{f(k)})|E|$
        %$|\phi^{-1}(S)\cap E|\geq (1-\frac{1}{f(k)})|E|$
        \item For each $X_i$, $i\in [k-|S|]$, $|X_i\cap S^*|=1$
         \item For each $i\in [k-|S|]$ and $E\in \mathcal{P}(S)$, $\gamma(i,E)=\lfloor \log_{1+\frac{1}{k}} \cov_{\phi^*}(S^*\cap X_i,\cA_E) \rfloor$
        \item For each $s\in S$ and $E\in \mathcal{P}(S)$, $\gamma(s,E)=\lfloor \log_{1+\frac{1}{k}} \cov_{\phi^*}(s,\cA_E) \rfloor$
        \item For each $E\in \mathcal{P}(S)$, $\pi(E)=\max_{s\in S}\cov_{\phi^*}(s,\cA_E)$
        % \item For each $i\in [k-|S|]$ and $E\in \mathcal{P}(S)$, $\gamma(i,E)=\lfloor \log_{1+\frac{1}{k}} |\phi^{-1}(S^*\cap X_i)\cap \cA_E| \rfloor$
        % \item For each $s\in S$ and $E\in \mathcal{P}(S)$, $\gamma(s,E)=\lfloor \log_{1+\frac{1}{k}} |\phi^{-1}(s)\cap \cA_E| \rfloor$
        % \item For each $E\in \mathcal{P}(S)$, $\pi(E)=\max_{s\in S}|\phi^{-1}(s)\cap \cA_E|$
    \end{enumerate}
    We also say $(S,X,\pi,\gamma)$ is good due to solution $S^*$.
\end{definition}

% \begin{observation}
% \label{observation:empty-good-tuple}
% $(\emptyset,X,.,.)$ is good if there exists a solution $S^*$ with $|X_i\cap S^*|=1$ for each $i\in [k]$.
% \end{observation}

\begin{lemma}
\label{lemma:annotated-d-hs}
    There exists an algorithm that takes as input an instance $\capinstance$, an annotated tuple $(S,X,\pi,\gamma)$ and in time $f(k)poly(n)$ either returns NO or a solution to $\capinstance$. Further, if $(S,X,\pi,\gamma)$ is good due to a solution $S^*$, $|S^*|\leq k$, it returns a solution of size at most $\frac{4}{3}|S^*|$.
\end{lemma}

\begin{theorem}
\label{theorem:main-alg}
    There exists an algorithm to \capdhs\ that takes as input an instance $\capinstance$ and in time $f(k)poly(n)$ either returns a solution of size at most $\frac{4}{3}k$ or determines there exists no solution of size at most $k$.
\end{theorem}

\begin{proof}
The algorithm does the following:
\begin{itemize}
    \item Construct a hash family $\mathcal{F}$ of sets $\{X_1,\cdots,X_k\}$.\todo{hash family}
    \item Construct a family $\mathcal{S}$ of sets $S\subseteq U$ having size at most $k$ satisfying $S\cap A\neq \emptyset$ for each $A\in \cA$ as follows:
    \begin{itemize}
        \item Order the sets in $\cA$ as $\cA=\{A_1,\cdots,A_{|A|}\}$
        \item \todo{greedy hs}
    \end{itemize}
    \item For each $\{X_1,\cdots,X_k\}\in \mathcal{F}$ and $S\in \mathcal{S}$ such that $X\cap S=\emptyset$ and for each $(S,X,\pi,\gamma)\in \cF_{S,X}$ use Lemma~\ref{lemma:annotated-d-hs} with $(S,X,\pi,\gamma)\in \cF_{S,X}$. If the algorithm returns a solution $S'$ of size at most $\frac{4}{3}k$, then return $S'$.  
    \item Return NO if no set was returned in the previous step.
\end{itemize}

Assume there exists a solution $S^*$ to $\capinstance$ of size at most $k$. Then by construction of $\mathcal{F}$, we know that there exists a $\{X_1,\cdots,X_k\}\in \mathcal{F}$ such that $X_i\cap S^*$ for each $i\in k$. By Observation~\ref{observation:empty-good-tuple}, we know that $(S,X,.,.)$ is good due to $S^*$. Thus invoking Lemma~\ref{lemma:annotated-d-hs} on $(S,X,.,.)$ returns a solution $S'$ to $\capinstance$ of size at most $\frac{4}{3}k$.
%
The time required to construct $\mathcal{F}$ is $ $\todo{}. Each call to Lemma~\ref{lemma:annotated-d-hs} runs in time $ $ and the Lemma is invoked $|\mathcal{F}|$ many times, thus the total runtime is $ $\todo.
\end{proof}

\subsection{Proof of Lemma~\ref{lemma:annotated-d-hs}}

% \begin{definition}
%    Given sets $S,X\subseteq U$ with $X\cap S=\emptyset$, let $\mathcal{F}_{S,X}$ denote the set of all possible annotated tuples $(S,X,\pi,\gamma)$.  
% \end{definition}
We start by providing our algorithm below. \\ \\
\textbf{Algorithm~2} \\
\textbf{Input:} An annotated tuple $(S,X,\pi,\gamma)$ and an instance $\capinstance$ \\
\textbf{Output: } $NO$ or a solution to $\capinstance$ of size at most $\frac{4}{3}k$
\begin{itemize}
    \item If $|S|=k$ and $S$ is a solution, return $S$ else return $NO$.
    \item For each $i\in [k-|S|]$ define
    $$X_i' \leftarrow \{x \in X_i: \mathsf{cap}(x) \geq \sum_{s \in S} \gamma(i,s) \text{ and } |\mathcal{A}_s \odot x| \geq \gamma(i,s) \text{ for all } s \in S\}$$
    \item For $i\in [k-|S|]$, $v\in X_i$ and $s\in S$ define $$\score(v,s):=\min\{|\cA_s \odot v|,\capa(v)-\sum_{s'\in S, s'\neq s} \gamma(i,s)\}$$
    \item For each $i\in [k-|S|]$, let $T(i,s)$ be the top $f(k)$ vertices of $X'_{i}$ when sorted in non-increasing order of $\score(v,s)$.
    \item For each pair of distinct functions $\tau_1: S\rightarrow [k-|S|]$ and $\tau_2:S\rightarrow [k-|S|]$ do:
    \begin{itemize}
        \item For each $i\in [k-|S|]$, construct the set $X''_i:=\bigcup_{s\in \tau_{1}^{-1}(i)}T(i,s)$ and let $X'':=\bigcup_{i\in [k-|S|]} X''_i$
        \item For each $i\in [k-1]$ and for each $v\in X''_i$
        \begin{itemize}
            \item Let $S':=S\cup \{v\}$ and $X':=X\setminus X_i$
            \item For each annotated tuple $(S',X',\pi',\gamma')\in \cF_{S',X'}$, apply Lemma~\ref{lemma:annotated-d-hs} on $(S',X',\pi',\gamma')$. If Lemma~\ref{lemma:annotated-d-hs}  returns a set of size at most $\frac{4}{3}k$ return it.
        \end{itemize}
    \item Construct the bipartite graph $H:=(S\uplus [k-s],E)$ where $E:=E_1\cup E_2$, $E_1:=\{(s,\tau_1(s)):s\in S\}$ and $E_2:=\{(s,\tau_2(s)):s\in S\}$.
    \item Find a set $D\subseteq [k-s]$ that dominates $S$ in $H$ such that $\{i\in [k-|S|]:|\tau_1^{-1}(i)|\geq 2\} \subseteq D$. 
    \item Construct a smallest size set $O\subseteq X''$ using Lemma~\ref{lemma:conflict-independent-set} such that:
    \begin{enumerate}
        \item $|O\cap X''_i|\geq 1$ for each $i\in [k-|S|]$
        \item $|O\cap X''_i|\geq 2$ for each $i\in D$
        %\item $|O\cap X''_i|\geq 2$ for each $i\in [k-|S|]$ such that $|\tau^{-1}(i)|\geq 2$.
        \item $O$ is $\frac{1}{k^2}$-conflict independent\todo{need stronger for bounds}
    \end{enumerate}
    \item Return $O\cup S$ if it is a solution of size at most $\frac{4}{3}k$
    \end{itemize}
\end{itemize}

It is clear that if the algorithm returns a set it is a solution of size at most $\frac{4}{3}k$. We now need to show that if $(S,X,\pi,\gamma)$ is good due to  a solution of size at most $k$, then the algorithm returns a solution of size at most $\frac{4}{3}k$.

From now, we fix $S^*$ be a solution of size at most $k$ due to which $(S,X,\pi,\gamma)$ is good. We prove that the algorithm returns a solution of size at most $\frac{4}{3}k$ by induction on the size of $S$. Base Case $|S|=k$: In this case  $S\subseteq S^*$ since $S^*$ is a solution due to which $(S,X,\pi,\gamma)$ is good. Further since $|S^*|\leq k$, $S^*=S$ and thus the algorithm returns $S$.

We now assume that the algorithm returns a solution of size at most $\frac{4}{3}k$ for all $S$ of size greater than $\ell$. We prove the claim for $|S|=\ell$. 

Let $X'=\bigcup_{i\in [k-|S|]} X'_i$. We observe that $X'$ filters out all vertices in $X$ that do not respect the estimate of coverage into each $E\in \cP$ according to $\gamma$. Formally, $(S,X',\pi,\gamma)$ is also good with respect to $S^*$ -- Recall that $(S,X',\pi,\gamma)$ is good due to $S^*$. Properties $1-3$ and $5-7$ in Definition~\ref{definition:good-tuple} depend only on $S,\gamma,\pi$ and so hold directly for $(S,X',\pi,\gamma)$ as well. By how we defined $X'_i$ and using properties $4$, $5$ and $6$ for $(S,X,\pi,\gamma)$, we can infer that $S^*\subseteq X'$ and $|X'_i\cap S^*|=1$ for each $i\in [k-|S|]$ proving property $2$ for $(S,X',\pi,\gamma)$. 

We now fix $\tau_1$ and $\tau_2$ according to $S^*$. Let,
$$v^*_i:=S^*\cap X'_i$$
$$\tau_1(s):=\max_{i\in[k-|S|]} |\phi^{-1}(v^*_i)\cap \cA_s|$$ $$\tau_2(s):=\max_{i\in[k-|S|]\setminus \tau_1(s)} |\phi^{-1}(v^*_i)\cap \cA_s|$$
%\textcolor{red}{Pick right $\tau_1$ and $\tau_2$ here}

Next we fix $X''_i$ for each $i\in [k-|S|]$ to be the one in the iteration of the algorithm with $\tau_1$ and $\tau_2$. Let $X'':=\bigcup_{i\in [k-s]}X''_i$. We divide our proof into two cases: $(i)$ $S^*\cap X''\neq \emptyset$ and $(ii)$ $S^*\cap X''=\emptyset$.

We first prove case $(i)$. Let $v\in S^*\cap X''$ and $v\in X''_i$. We define $S':=S^*\cup\{v\}$ and $Y:=X\setminus X_i$. Since $(S,X,\pi,\gamma)$ is good due to $S^*$, there exists an annotated tuple $(S',Y,\pi',\gamma')$ that is good with respect to $S^*$. The algorithm goes over every annotated tuple in $\cF_{S',Y}$ and thus calls Lemma~\ref{lemma:annotated-d-hs} on $(S',Y,\pi',\gamma')$. By induction since $|S'|>|S|$, this recursive call returns a solution of size at most $\frac{4}{3}k$.
%
To complete our proof, we need to prove the claim for case $(ii)$. For this, we first show $S\cup O$ is a solution.
\begin{lemma}
If $S^*\cap X''=\emptyset$, then $S\cup O$ is a solution to $\capinstance$.


\end{lemma}
\begin{proof}
Let $\phi^*:\cA\rightarrow S^*$ be an assignment of $\mathcal{A}$ to $S^*$. 
%
For the proof we construct an assignment $\phi:\cA \rightarrow S\cup O$ such that for each $x\in S\cup O$, $\cov_{\phi}(x,\cA)\leq \capa(x)$. We first describe how to construct the assignment.

Recall that $O\subseteq X''$. For each $o\in O$ such that $o\in X''_i$

Define $Y_o$, then $Y'_o$

For each $o\in O$ and $A\in Y'_o$, define $\phi(A)=o$. 

\begin{claim}
    For each $s\in S$, $\cov_{\phi}(O,\cA_s)\geq \cov_{\phi^*}(S^*\setminus S,\cA_s)$
\end{claim}
\begin{proof}
    
\end{proof}
\begin{claim}
    For each $E\in \cP(S)$, if $\cov_{\phi}($
\end{claim}
Let $s\in S$ and let $\cov_{\phi^*}(S^*\setminus S,\cA_s)$

\begin{claim} For each $E\in \cP(S)$, $\cov_{\phi^*}(S,E)\geq (1-\frac{1}{f(k)})|E|$
\end{claim}
%
% We first prove that for each $E\in \cP$, $S$ covers a large portion of $E$ in $S^*$, i.e $|\phi^{-1}(S)\cap E|\geq (1-\frac{1}{f(k)})|E|$.
% \begin{lemma}
%     If $S^*\cap X''=\emptyset$ then for each $E\in \cP(S)$, $|\phi^{-1}(S)\cap E|\geq (1-\frac{1}{f(k)})|E|$
% \end{lemma}
% \begin{proof}
%     Suppose not, then there exists $E$ such that $|\phi^{-1}(S)\cap E|< (1-\frac{1}{f(k)})|E|$. Let $i=\tau_1(\pi(E))$ and $v_i=S^*\cap X_i$, then this fact long with the definition of $\tau_1$ ensures $|\phi^{-1}(v_i)\cap E|\geq \frac{1}{k}\frac{1}{f(k)}|E|$. Since $S^*\cap X''=\emptyset$, $v\notin X''_i$. By definition of $score$ \textcolor{red}{Note we need argument for E but holds only for stars A_s}
% \end{proof}


\end{proof}

\begin{lemma}
$|S\cup O|\leq \frac{4}{3}$    
\end{lemma}
\begin{proof} Let $s=|S|$, we divide the analysis into two cases: (i) $k-s<2s$ and (ii) $k-s\geq 2s$. First observe that $|S \cup O|=|S|+k-|S|+|D|=k+|D|$.
For case (i) we use that $|D|\leq \frac{1}{3}(|S|+k-|S|)$ by Lemma~\ref{}. Here $|S\cup O|\leq k+|D|\leq k+1/3(|S|+k-|S|)\leq 4k/3$.
.
    \item \textbf{Case 2 ($r\geq 2s$)}:
    In this case, we can find a dominating set of size $s$. Therefore, we have the following upper bound on the size of the found solution: $|S| + r + |D| \leq k + s \leq \frac{4k}{3}$.
\end{proof}

% \begin{lemma}Let $G=R\uplus B$ be an instance of \textsc{Red Blue Dominating Set} with $|R|=r$ and $|B|=b$ satisfying $r<2b$ and $deg(v)\geq 2$, $\forall v \in B$. Then there exists a red-blue dominating set $D\subseteq R$ of size at most $\frac{1}{3}(b+r)$ that can be found in polynomial time.
% \end{lemma}


% \begin{definition}
%     Let $(S,X,\pi,\gamma)$ be a good tuple due to a solution $S^*$, then a pair of functions $(\tau_1,\tau_2)$ where $\tau_1:S\rightarrow [k-|S|]$ and $\tau_2:S\rightarrow [k-|S|]$ is good if:
%     \begin{itemize}
%         \item For each $s\in S$, 
%     \end{itemize}
% \end{definition}


\subsection{Conflict Independence}
We use the notion of conflict independence crucially in our result.

\begin{definition}
Two element $a,b\in U$ are said to be conflict independent if $a$    
\end{definition}

\begin{lemma}
\label{lemma:conflict-independent-set}
    Given a set $X\subseteq U$, $X=X_1\uplus \cdots \uplus X_{\ell\leq k}$ with $|X_i|\geq $, one can in polynomial time find sets $Y_1,\cdots,Y_\ell$ such that $Y_i\subseteq X_i$, $Y_i\geq 2$ and $\cup_{i\in [\ell]}Y_i$ is $\frac{1}{k^2}$-independent.
\end{lemma}

\section{Conclusion}
Also works for partial $d$-HS with same ratio by the $d$ to $d+1$ reduction.

==> capdhs_preamble.tex <==
\usepackage{setspace}
\usepackage{subcaption}
\usepackage{enumerate}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{tcolorbox}
%\usepackage[hidelinks]{hyperref}
\usepackage{amssymb}
\usepackage{multirow}
\usepackage{geometry}
\usepackage{soul}
\usepackage{colortbl}
\usepackage{wrapfig}
\usepackage{algorithm}
\usepackage{algorithmicx}
%\usepackage{amsthm}
\usepackage{todonotes}
\usepackage{mathtools}
\usepackage{mathrsfs}
\usepackage{thmtools} 

\newcommand{\dist}{{\sf dist}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%paper specific%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\capinstance}
{(U,\mathsf{cap},\mathcal{A})}
\newcommand{\capdhs}{\textsc{Capacitated $d$-Hitting Set}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\capa}{\mathsf{cap}}
\newcommand{\score}{\mathsf{score}}
\newcommand{\covp}{\mathsf{cov}_{\phi}}
\newcommand{\cov}{\mathsf{cov}}
\newcommand{\sbra}[1]{\left[ #1 \right]}
\newcommand{\cbra}[1]{\left\{ #1 \right\}}
\newcommand{\bin}{\{0,1\}}
\newcommand{\opt}{\mathsf{OPT}}

\newcommand{\first}{TOP}

\newcommand{\val}{\mathsf{val}}
\newcommand{\vala}{?_1}
\newcommand{\valb}{?_2}
\algtext*{EndWhile}% Remove "end while" text
\algtext*{EndIf}% Remove "end if" text
\algtext*{EndFor}% Remove "end for" text
\algtext*{EndProcedure}
\algtext*{EndFunction}


\newtheorem{definition}[lemma]{Definition}
\newtheorem{observation}[lemma]{Observation}
\newtheorem{claim}[lemma]{Claim}

==> intro.tex <==
%!TEX root = main.tex
A vertex-deletion problem takes as input a graph $G$, and aims to delete from $G$ a minimum number of vertices such that the resulting graph satisfies some property.
In many vertex-deletion problems, the desired properties can be expressed as excluding a finite set of ``forbidden'' structures.
This motivates the so-called \textsc{$\mathcal{F}$-Hitting} problem.
Formally, for a finite set $\mathcal{F}$ of graphs (which represent the forbidden structures), the \textsc{$\mathcal{F}$-Hitting} problem is defined as follows.

\begin{tcolorbox}[colback=gray!5!white,colframe=gray!75!black]
        \textsc{$\mathcal{F}$-Hitting} \hfill \textbf{Parameter:} $k$
        \vspace{0.1cm} \\
        \textbf{Input:} A graph $G$ of $n$ vertices (taken from some graph class $\mathcal{G}$) and an integer $k \in \mathbb{N}$.
        \vspace{0.1cm} \\
        \textbf{Goal:} Compute a set $S \subseteq V(G)$ of vertices such that $|S| \leq k$ and $G - S$ does not contain any graph in $\mathcal{F}$ as a subgraph.
        %Return NO if such a set does not exist.
\end{tcolorbox}

As a generic problem, \textsc{$\mathcal{F}$-Hitting} subsumes many fundamental vertex-deletion problems that have been well-studied in the literature, such as \textsc{Vertex Cover}, \textsc{Path Transversal}~\cite{brevsar2013vertex,gupta2019losing,lee2017partitioning}, \textsc{Short Cycle Hitting}~\cite{groshaus2009cycle,lokshtanov2022subexponential,lokshtanov2023framework,pilipczuk2011problems}, \textsc{Component Order Connectivity}~\cite{drange2016computational,gross2013survey,kumar20172lk}, \textsc{Degree Modulator}~\cite{betzler2012bounded,ganian2021structural,gupta2019losing}, \textsc{Treedepth Modulator}~\cite{bougeret2019much,eiben2022lossy,gajarsky2017kernelization}, \textsc{Clique Hitting}~\cite{fiorini2018approximability}, \textsc{Biclique Hitting}~\cite{goldmann2021parameterized}, etc.
We present in the appendix detailed descriptions of these problems as well as their background (see also the work~\cite{lokshtanov2023hitting}).
%~\cite{aprile2021tight,betzler2012bounded,bougeret2019much,brevsar2013vertex,drange2016computational,eiben2022lossy,fiorini2020improved,fiorini2018approximability,gajarsky2017kernelization,ganian2021structural,goldmann2021parameterized,gross2013survey,groshaus2009cycle,gupta2019losing,kumar20172lk,lee2017partitioning,lokshtanov2022subexponential,lokshtanov2023framework,pilipczuk2011problems,you2017approximate}



On general graphs (i.e., when the graph class $\mathcal{G}$ contains all graphs), the complexity of \textsc{$\mathcal{F}$-Hitting} is well-understood.
For any (finite) $\mathcal{F}$, the problem admits a simple branching algorithm with running time $2^{O(k)} \cdot n^{O(1)}$~\cite{Cai96}.
On the other hand, by the seminal result of Lewis and Yannakakis~\cite{lewis1980node}, \textsc{$\mathcal{F}$-Hitting} cannot be solved in $2^{o(k)} \cdot n^{O(1)}$ time or even $2^{o(n)}$ time for any nontrivial\footnote{Here ``nontrivial'' means that there exist infinitely many graphs that contain some graph in $\mathcal{F}$ as a subgraph and also infinitely many graphs that do not contain any graph in $\mathcal{F}$ as a subgraph. Note that if $\mathcal{F}$ is trivial, then \textsc{$\mathcal{F}$-Hitting} can be trivially solved in polynomial time.} $\mathcal{F}$, assuming the Exponential-Time Hypothesis.
However, this does not rule out the existence of subexponential (parameterized) algorithms for \textsc{$\mathcal{F}$-Hitting} on restrictive graph classes.
In fact, many special cases of \textsc{$\mathcal{F}$-Hitting} have been solved in subexponential time on various graph classes.
For example, \textsc{Vertex Cover}, the simplest (nontrivial) case of \textsc{$\mathcal{F}$-Hitting}, was known to have $2^{O(\sqrt{k})} \cdot n^{O(1)}$-time algorithms on many graph classes, such as planar graphs, minor-free graphs, unit-disk graphs, map graphs, and disk graphs~\cite{DemaineFHT05,ErlebachJS05,FominLPSZ19,FominLS18,FominLP0Z19,lokshtanov2022subexponential}.
Some other cases, such as \textsc{Path Transversal}, \textsc{Triangle Hitting}, \textsc{Component Order Connectivity}, etc., were also known to admit subexponential parameterized algorithms on specific graph classes, mostly planar graphs, minor-free graphs, and (unit-)disk graphs~\cite{DemaineFHT05,FominLPSZ19,FominLS18,lokshtanov2022subexponential}.
Nevertheless, there has not been a comprehensive study on subexponential algorithms for the general \textsc{$\mathcal{F}$-Hitting} problem.

In this paper, we systematically study the \textsc{$\mathcal{F}$-Hitting} problem on a broad family of graph classes, in the context of subexponential parameterized algorithms.
We show that on almost all common graph classes where subexponential algorithms have been well-studied, \textsc{$\mathcal{F}$-Hitting} admits a subexponential parameterized algorithm for any $\mathcal{F}$.

\paragraph{Other related work on \textsc{$\mathcal{F}$-Hitting}.}
The general \textsc{$\mathcal{F}$-Hitting} problem has been studied on graphs of bounded treewidth by Cygan et al. \cite{cygan2017hitting}, who gave FPT algorithms (parameterized by treewidth) and lower bounds for the problem and its variants.
Very recently, Dvo{\v{r}}{\'a}k et al.~\cite{lokshtanov2023hitting} studied \textsc{$\mathcal{F}$-Hitting} in the perspective of approximation, showing that the local-search approach of Har-Peled and Quanrud~\cite{har2017approximation} for \textsc{Vertex Cover} and \textsc{Dominating Set} on graph classes of polynomial expansion can be extended to obtain PTASes for \textsc{$\mathcal{F}$-Hitting} as well.
They also gave a $(1+\varepsilon)$-approximation reduction from the problem on any bounded-expansion graph class to the same problem on bounded degree graphs within the class, resulting in lossy kernels for the problem.
Finally, \textsc{$\mathcal{F}$-Hitting} is a special case of \textsc{$d$-Hitting Set}, and hence the algorithms for \textsc{$d$-Hitting Set}~\cite{CyganFKLMPPS15,williamson2011design} also apply to \textsc{$\mathcal{F}$-Hitting}.
However, as the set system considered in \textsc{$\mathcal{F}$-Hitting} is implicitly defined and can have size $n^{O(\gamma)}$ where $\gamma = \max_{F \in \mathcal{F}} |V(F)|$, transferring the algorithms for \textsc{$d$-Hitting Set} to \textsc{$\mathcal{F}$-Hitting} usually results in an overhead of $n^{O(\gamma)}$.

\subsection{Our result}

Our main result is a general framework to design subexponential parameterized algorithms for \textsc{$\mathcal{F}$-Hitting}.
In fact, our framework applies to the weighted version of \textsc{$\mathcal{F}$-Hitting}, where the vertices are associated with weights and we want to find the solution with the minimum total weight.

\begin{tcolorbox}[colback=gray!5!white,colframe=gray!75!black]
        \textsc{Weighted $\mathcal{F}$-Hitting} \hfill \textbf{Parameter:} $k$
        \vspace{0.1cm} \\
        \textbf{Input:} A graph $G$ of $n$ vertices (taken from some graph class $\mathcal{G}$) together with a weight function $w:V(G) \rightarrow \mathbb{R}_{\geq 0}$, and an integer $k \in \mathbb{N}$.
        \vspace{0.1cm} \\
        \textbf{Goal:} Compute a minimum-weight (under the function $w$) set $S \subseteq V(G)$ of vertices such that $|S| \leq k$ and $G - S$ does not contain any graph in $\mathcal{F}$ as a subgraph.
        %Return NO if such a set does not exist.
\end{tcolorbox}

To present our results, we need to define the graph classes to which our framework applies.
We define these graph classes in the language of \textit{balanced separators}, which serve as a key ingredient in many efficient graph algorithms.
We say a graph $G$ admits \textit{balanced $(\eta,\mu,\rho)$-separators} if for every induced subgraph $H$ of $G$, there exists $S \subseteq V(H)$ of size at most $\eta \cdot \omega^\mu(H) \cdot |V(H)|^\rho$ such that every connected component of $H - S$ contains at most $\frac{1}{2} |V(H)|$ vertices, where $\omega(H)$ denotes the size of a maximum clique in $H$.
Throughout this paper, we denote by $\mathcal{G}(\eta,\mu,\rho)$ the class of all graphs admitting balanced $(\eta,\mu,\rho)$-separators.
Trivially, every graph admits balanced $(1,0,1)$-separators.
Thus, we only consider the case $\rho < 1$.
Our framework results in the following theorem.

\begin{theorem} \label{thm-main}
    Let $\mathcal{G} \subseteq \mathcal{G}(\eta,\mu,\rho)$ where $\eta,\mu \geq 0$ and $0 \leq \rho < 1$.
    Also, let $\mathcal{F}$ be a finite set of graphs.
    Then there exists a constant $c < 1$ (depending on $\eta$, $\mu$, $\rho$, and $\mathcal{F}$) such that the \textsc{Weighted $\mathcal{F}$-Hitting} problem on $\mathcal{G}$ can be solved in $2^{O(k^c)} \cdot n^4$ time.
\end{theorem}

We now briefly discuss why the graph classes in Theorem~\ref{thm-main} are interesting.
The sub-classes of $\mathcal{G}(\eta,0,\rho)$ for $\rho < 1$ are known as graph classes with \textit{strongly sublinear separators}.
Dvo\v{r}\'{a}k and Norin~\cite{DorakN2016} showed that these classes are equivalent to graph classes of \textit{polynomial expansion}, which is a well-studied special case of \textit{bounded-expansion} graph classes introduced by Ne{\v{s}}et{\v{r}}il and De Mendez \cite{nevsetvril2008grad,nevsetvril2008grad2}.
Important examples of polynomial-expansion graph classes include planar graphs, bounded-genus graphs, minor-free graphs, $k$-nearest neighbor graphs~\cite{miller1997separators}, greedy Euclidean spanners~\cite{le2022greedy}, etc.
For a general $\mu \geq 0$, the classes $\mathcal{G}(\eta,\mu,\rho)$ with $\rho < 1$ in addition subsume a broad family of geometric intersection graphs.
A \textit{geometric intersection graph} is defined by a set of geometric objects in a Euclidean space, where the objects are the vertices and two vertices are connected by an edge if their corresponding objects intersect.
Intersection graphs of any fat objects (i.e., convex geometric objects whose diameter-width ratio is bounded) and intersection graphs of pseudo-disks (i.e., topological disks in the plane satisfying that the boundaries of every pair of them are either disjoint or intersect twice) admit balanced $(\eta,\mu,\rho)$-separators for $\rho < 1$~\cite{lokshtanov2023hitting,miller1997separators}.
These two families, in turn, cover many interesting cases of geometric intersection graphs, such as (unit-)disk graphs, ball graphs, hypercube graphs, map graphs, intersection graphs of non-crossing rectangles, etc.
To summarize, the graph classes $\mathcal{G}(\eta,\mu,\rho)$ for $\rho < 1$ cover many common graph classes on which subexponential algorithms have been well-studied.
%Graph classes of single-exponential expansion is a special case of \textit{bounded-expansion} graph classes introduced by Ne{\v{s}}et{\v{r}}il and De Mendez \cite{nevsetvril2008grad,nevsetvril2008grad2}.
%subexponential parameterized algorithms for \textsc{Weighted $\mathcal{F}$-Hitting} on all $\mathcal{G}(\eta,\mu,\rho)$ with $\rho < 1$.

It is natural to ask whether the result in Theorem~\ref{thm-main} can be extended to \textsc{$\mathcal{F}$-Hitting} with an infinite $\mathcal{F}$.
A typical example is \textsc{Feedback Vertex Set}, where $\mathcal{F}$ consists of all cycles.
Unfortunately, this seems impossible.
Indeed, it was known~\cite{FominLS18} that \textsc{Feedback Vertex Set} does not admit subexponential FPT algorithms on unit-ball graphs with bounded ply, which belong to the class $\mathcal{G}(\eta,0,\rho)$ for some $\eta$ and $\rho < 1$.
Another extension one may consider is to the \textsc{Induced $\mathcal{F}$-Hitting} problem, where the goal is to hit all \textit{induced} subgraphs of $G$ that are isomorphic to some graph in $\mathcal{F}$.
Again, Theorem~\ref{thm-main} is unlikely to hold for \textsc{Induced $\mathcal{F}$-Hitting}.
Indeed, when $\mathcal{F}$ consists of a single edgeless graph of $p$ vertices, \textsc{Induced $\mathcal{F}$-Hitting} (with $k=0$) is equivalent to detecting an independent set of size $p$ and thus an algorithm for \textsc{Induced $\mathcal{F}$-Hitting} on a graph class $\mathcal{G}$ with running time as in Theorem~\ref{thm-main} would imply an FPT algorithm for \textsc{Independent Set} on $\mathcal{G}$.
But \textsc{Independent Set} is W[1]-hard even on unit-disk graphs~\cite{CyganFKLMPPS15}.
Note that while this rules out the possibility of extending Theorem~\ref{thm-main} to \textsc{Induced $\mathcal{F}$-Hitting}, it might still be possible to obtain a weaker bound of $2^{O(k^c)} \cdot n^{f(\mathcal{F})}$ for $c<1$ and some function $f$, which we leave as an interesting open question for future study.
\medskip

\noindent
\textbf{Remark.}
The quartic dependency on $n$ of the running time of our algorithms can probably be improved, and we have not made attempt to optimize it in this paper.

%\medskip
%\paragraph{Techniques.}
\subsection{Building blocks}
Our framework is built on two technical components developed in this paper, both of which are of independent interest.
The first one is a novel fixed-parameter tractable (FPT) algorithm for \textsc{Subgraph Isomorphism} on the aforementioned graph classes.
For graphs $F$ and $G$, an \textit{$F$-copy} in $G$ is a pair $(H,\pi)$ where $H$ is a subgraph of $G$ and $\pi:V(H) \rightarrow V(F)$ is an isomorphism between $H$ and $F$.
The \textsc{Subgraph Isomorphism} problem is defined as follows.

\begin{tcolorbox}[colback=gray!5!white,colframe=gray!75!black]
        \textsc{Subgraph Isomorphism} \hfill \textbf{Parameter:} $t$
        \vspace{0.1cm} \\
        \textbf{Input:} A graph $G$ of $n$ vertices (taken from some graph class $\mathcal{G}$) and a graph $F$ of $t$ vertices.
        \vspace{-0.4cm} \\
        %\textbf{Goal:} Compute a subgraph $H' \subseteq G$ and an isomorphism $f: V(H) \rightarrow V(H')$ between $H$ and $H'$ such that $f(v) \in R_v$ for all $v \in V(H)$.
        \textbf{Goal:} Find an $F$-copy $(H,\pi)$ in $G$.
\end{tcolorbox}

FPT algorithms for \textsc{Subgraph Isomorphism} on graph classes of bounded expansion are well-known \cite{dvovrak2013testing,nevsetvril2006linear,nevsetvril2008grad2}, and it is not difficult to extend them to the classes $\mathcal{G}(\eta,\mu,\rho)$ for $\rho < 1$.
Unfortunately, while the running times of these algorithms are linear in $n$, they have extremely heavy dependency on the parameter $t$.
Even on graph classes of polynomial expansion, the time complexity of these algorithms is at least double-exponential in $t$.
When detecting a \textit{fixed} pattern $F$ (i.e., $t$ is a constant), this does not matter too much.
However, in our framework for \textsc{$\mathcal{F}$-Hitting}, we need to find subgraphs of size related to the parameter $k$ (more precisely, $t = k^{\varepsilon}$ for a small constant $\varepsilon > 0$).
Thus, we cannot afford using the existing algorithms for \textsc{Subgraph Isomorphism}.
%even on graph classes of polynomial expansion.

We give a single-exponential\footnote{Throughout this paper, a single-exponential function refers to a function of the form $f(x) = 2^{x^{O(1)}}$.} FPT algorithm for \textsc{Subgraph Isomorphism} on graph classes $\mathcal{G}(\eta,\mu,\rho)$ with $\rho < 1$ (and others).
In fact, our algorithm can be applied to any graphs and has good running time on certain graph classes.
%any graph classes $\mathcal{G}(\eta,\mu,\rho)$ where $\rho<1$ and any graph class of single-exponential expansion.
We say a collection $\mathcal{S}$ of subgraphs of $G$ is a \textit{$t$-exhaustive} subgraph list if for any subgraph $H \subseteq G$ of at most $t$ vertices, there exists $H' \in \mathcal{S}$ such that $H' \simeq H$ (i.e., $H'$ is isomorphic to $H$).
We prove the following theorem, where $b_t(G) = |E(H)|/|V(H)|$ for a densest $t$-vertex subgraph $H \subseteq G$ and $\textnormal{wcol}_t(G,\sigma)$ is the $t$-th weak coloring number of $G$ under the ordering $\sigma$ (see Section~\ref{sec-pre} for the formal definition).

\begin{restatable}{theorem}{sublist} \label{thm-sublist}
    Given a graph $G$ of $n$ vertices, an ordering $\sigma$ of the vertices of $G$, and an integer $t \in \mathbb{N}$, one can compute in $(2^{b_t(G)}+\textnormal{wcol}_t(G,\sigma))^{O(t)} \cdot n$ time a $t$-exhaustive subgraph list $\mathcal{S}$ of $G$.
    The size of $\mathcal{S}$ is also bounded by $(2^{b_t(G)}+\textnormal{wcol}_t(G,\sigma))^{O(t)} \cdot n$.
\end{restatable}

Note that the above theorem directly gives an algorithm for \textsc{Subgraph Isomorphism} with the same asymptotic time complexity: we simply compute the $t$-exhaustive subgraph list $\mathcal{S}$ of $G$ and check if the pattern graph $F$ is isomorphic to any one in $\mathcal{S}$.
Combining the theorem with known algorithms for computing a good ordering $\sigma$, we obtain single-exponential FPT algorithms for \textsc{Subgraph Isomorphism} on any graph classes $\mathcal{G}(\eta,\mu,\rho)$ with $\rho<1$ and any graph class of \textit{single-exponential expansion}, a special case of bounded-expansion graph classes.

\begin{corollary}[Corollaries~\ref{cor-subisoclique} and~\ref{cor-subisoexpexp} combined] \label{cor-subisocombined}
    The following statements hold.
    \begin{itemize}
        \item Let $\mathcal{G} \subseteq \mathcal{G}(\eta,\mu,\rho)$ where $\eta,\mu \geq 0$ and $0 \leq \rho < 1$.
        Then \textsc{Subgraph Isomorphism} on $\mathcal{G}$ can be solved in $t^{O(t^3)} \cdot n^4$ time.
        %When $\mu = 0$, the running time can be improved to $t^{O(t)} \cdot n^4$
        \item Let $\mathcal{G}$ be a graph class of single-exponential expansion.
        Then \textsc{Subgraph Isomorphism} on $\mathcal{G}$ can be solved in $2^{t^{O(1)}} \cdot n^4$ time.
    \end{itemize}
\end{corollary}

Interestingly, graph classes of single-exponential expansion, though being more restrictive than bounded-expansion ones, cover many important cases of bounded-expansion graph classes, including graphs with bounded queue number~\cite{nevsetvril2012characterisations}, graphs with bounded stack number~\cite{nevsetvril2012characterisations}, graphs of bounded degree~\cite{nevsetvril2008grad}, Erd{\"o}s-R{\'e}nyi random graphs~\cite{nevsetvril2012characterisations}, and of course all polynomial-expansion graph classes.
%On graph classes with polynomial weak coloring numbers, Theorem~\ref{thm-sublist} implies an even more efficient algorithm for \textsc{Subgraph Isomorphism}, which runs in $t^{O(t)} \cdot n^4$ time.

The second technical component of our framework, which is our main technical contribution, is an intricate branching algorithm that reduces in subexponential FPT time an instance of \textsc{$\mathcal{F}$-Hitting} (on the aforementioned graph classes) to multiple general hitting-set instances, where the Gaifman graph of each instance has treewidth sublinear in $k$.
We say a set $S \subseteq V(G)$ is an \textit{$\mathcal{F}$-hitting set} of $G$ if $G - S$ does not contain any graph in $\mathcal{F}$ as a subgraph.
Let $\mathcal{X}$ be a collection of sets (in which the elements belong to the same universe).
The \textit{Gaifman graph} of $\mathcal{X}$ is the graph with vertex set $\bigcup_{X \in \mathcal{X}} X$ where two vertices $u$ and $v$ are connected by an edge if $u,v \in X$ for some $X \in \mathcal{X}$.
We say a set $S$ \textit{hits} $\mathcal{X}$ if $S \cap X \neq \emptyset$ for all $X \in \mathcal{X}$.
We prove the following theorem.

\begin{restatable}{theorem}{branching} \label{thm-subtwbranch}
%Let $\mathcal{G}$ be a graph class of polynomial expansion, 
Let $\mathcal{G} \subseteq \mathcal{G}(\eta,\mu,\rho)$ where $\eta,\mu \geq 0$ and $\rho < 1$.
Also, let $\mathcal{F}$ be a finite set of graphs.
Then there exists a constant $c < 1$ (depending on $\eta$, $\mu$, $\rho$, and $\mathcal{F}$) such that for a given graph $G \in \mathcal{G}$ of $n$ vertices and a parameter $k \in \mathbb{N}$, one can construct in $2^{O(k^c)} \cdot n^4$ time $m = 2^{O(k^c)}$ collections $\mathcal{X}_1,\dots,\mathcal{X}_m$ of subsets of $V(G)$ satisfying the following conditions.
\begin{itemize}
    \item For any $S \subseteq V(G)$ with $|S| \leq k$, $S$ is an $\mathcal{F}$-hitting set of $G$ iff $S$ hits $\mathcal{X}_i$ for some $i \in [m]$.
    \item The Gaifman graph of $\mathcal{X}_i$ has treewidth $O(k^c)$, for all $i \in [m]$.
\end{itemize}
\end{restatable}

The subexponential implementation of the algorithm in Theorem~\ref{thm-subtwbranch} relies heavily on our single-exponential algorithm for \textsc{Subgraph Isomorphism} in Corollary~\ref{cor-subisocombined}.
The proof of Theorem~\ref{thm-subtwbranch} introduces interesting combinatorial results (e.g., Lemma~\ref{lem-twGaifman}) for the set systems considered in the \textsc{$\mathcal{F}$-Hitting} problem (i.e. the vertex sets of all subgraphs isomorphic to some graph in $\mathcal{F}$), which might be useful for understanding the structure of such set systems.

Provided Theorem~\ref{thm-subtwbranch}, it is easy to prove our main result in Theorem~\ref{thm-main}.
Given an instance $(G,w,k)$ of \textsc{Weighted $\mathcal{F}$-Hitting} where $G \in \mathcal{G} \subseteq \mathcal{G}(\eta,\mu,\rho)$ for $\rho < 1$, we simply compute the collections $\mathcal{X}_1,\dots,\mathcal{X}_m$ in Theorem~\ref{thm-subtwbranch} for the graph $G$.
Then we compute a minimum-weight (under the weight function $w$) hitting set $S_i$ for each $\mathcal{X}_i$ satisfying $|S_i| \leq k$, which can be done in $2^{O(k^c)} \cdot n$ time (where $c<1$ is the constant in Theorem~\ref{thm-subtwbranch}) by standard dynamic programming, because the treewidth of the Gaifman graph of $\mathcal{X}_i$ is $O(k^c)$.
Finally, we return the set $S_i$ with the minimum total weight among $S_1,\dots,S_m$.
The first condition in Theorem~\ref{thm-subtwbranch} guarantees that $S_i$ is an optimal solution for the \textsc{Weighted $\mathcal{F}$-Hitting} instance.
The overall running time is $2^{O(k^c)} \cdot n^4$.

\paragraph{Organization.}
In Section~\ref{sec-overview}, we give an informal overview of our proofs.
In Section~\ref{sec-pre}, we give the formal definitions of the basic notions used in this paper.
Sections~\ref{sec-subisom} and~\ref{sec-branching} present the proofs of Theorems~\ref{thm-sublist} and~\ref{thm-subtwbranch}, respectively.
Finally, in Section~\ref{sec-subhit}, we prove Theorem~\ref{thm-main}.



==> preliminary.tex <==

%\todo[inline]{Definition $\sigma[i],\sigma[i,j]$ for an ordering $\sigma$}

\paragraph{Basic notations.}
We use $\mathbb{N}$ to denote the set $\{1,2,3,\ldots\}$, and write $[n]=\{1,2,\ldots,n\}$ for short.
For a graph $G$, the notations $V(G)$ and $E(G)$ denote the set of vertices and the set of edges in $G$, respectively.
For a vertex subset $S\subseteq V(G)$, $N_G(S)=\{u\in V(G)\setminus S~\colon~ (u,x)\in E(G) \mbox{ for some }x\in S\}$ and 
$N_G[S]=N_G(S)\cup S$. 
%\paragraph{Subgraphs and induced subgraphs.}
%Let $G = (V,E)$ be a graph.
A \textit{subgraph} of $G$ is a graph $G' = (V',E')$, denoted by $G'\subseteq G$, where $V' \subseteq V(G)$ and $E' \subseteq E(G)$.
The graph $G'$ is an {\em induced subgraph} of $G$ if $E'=\{(u,v)\in E(G)~\colon~u\in V' \mbox{ and } v\in V'\}$. 
For a set $V \subseteq V(G)$, the notation $G[V]$ denotes the subgraph of $G$ induced by $V$.
The notation $\omega(G)$ denotes the size (i.e., number of vertices) of a maximum clique in $G$.
Two graphs $G$ and $G'$ are \textit{isomorphic}, denoted by $G \simeq G'$, if there exists a bijective map $\pi:V(G) \rightarrow V(G')$ such that $(u,v) \in E(G)$ iff $(f(u),f(v)) \in E(G')$.
The function $\pi$ is called an \textit{isomorphism} between $G$ and $G'$.
For graphs $F$ and $G$, an \textit{$F$-copy} in $G$ is a pair $(H,\pi)$ where $H \subseteq G$ and $\pi: V(H) \rightarrow V(F)$ is an isomorphism between $H$ and $F$.
We say $G$ is \textit{$F$-free} if there is no $F$-copy in $G$.
For a set $\mathcal{F}$ of graphs, $G$ is \textit{$\mathcal{F}$-free} if it is $F$-free for all $F \in \mathcal{F}$.

\begin{lemma} \label{lem-isom}
    Let $G$ and $G'$ be two graphs, and $\pi:V(G) \rightarrow V(G')$ be a bijective map.
    Also, let $V_1,\dots,V_r \subseteq V(G)$ and $V_i' = f(V_i)$ for $i \in [r]$.
    If $G = \bigcup_{i=1}^r G[V_i]$, $G' = \bigcup_{i=1}^r G'[V_i']$, and $\pi_{|V_i}$ is an isomorphism between $G[V_i]$ and $G'[V_i']$ for all $i \in [r]$, then $\pi$ is an isomorphism between $G$ and $G'$.
\end{lemma}
\begin{proof}
Let $u,v$ be two distinct vertices in $V(G)$. Let $u'=f(u)$ and $v'=f(v)$. Notice that $(u,v)\in E(G)$ if and only if there is an integer $i\in [r]$ such that $(u,v)\in E(G_i)$. Thus, since $\pi_{|V_j}$ is an isomorphism between $G[V_j]$ and $G'[V_j']$ for all $j \in [r]$, $(u,v)\in E(G)$ if and only if $(u',v')\in E(G')$. This completes the proof of the lemma.      
\end{proof}

\paragraph{Hitting set and Gaifman graphs.}
Let $\mathcal{A}$ be a collection of sets whose elements belong to a common universe $U$.
A set $S \subseteq U$ \textit{hits} $\mathcal{A}$ (or is a \textit{hitting set} of $\mathcal{A}$) if $S \cap A \neq \emptyset$ for all $A \in \mathcal{A}$.
The \textit{Gaifman graph} of $\mathcal{A}$ is a graph with vertex set $\bigcup_{A \in \mathcal{A}} A$ where two vertices $u$ and $v$ are connected by an edge if $u,v \in A$ for some $A \in \mathcal{A}$.
For a graph $G$ and a set $\mathcal{F}$ of graphs, an \textit{$\mathcal{F}$-hitting set} of $G$ is a hitting set of $\{V(H): H \subseteq G \text{ and } H \simeq F \text{ for some } F \in \mathcal{F}\}$.
Equivalently, an $\mathcal{F}$-hitting set of $G$ is a set $S \subseteq V(G)$ such that $G-S$ is $\mathcal{F}$-free.

\paragraph{Sunflowers and representative sets.}
Let $V_1,\dots,V_r$ be sets whose elements belong to a common universe $U$.
We say $V_1,\dots,V_r$ form a \textit{sunflower} if $V_1 \backslash X,\dots,V_r \backslash X$ are disjoint, where $X = \bigcap_{i=1}^r V_i$.
We call $X$ the \textit{core} of the sunflower.
\begin{lemma}[sunflower lemma] \label{lem-sunflower}
Let $\mathcal{A}$ be a collection of sets whose sizes are at most $p$.
If $|\mathcal{A}| \geq (r-1)^p \cdot p!$, then there exist $r$ sets in $\mathcal{A}$ which form a sunflower.
\end{lemma}

For a collection $\mathcal{A}$ of sets whose elements belong to a common universe $U$, a \textit{$q$-representative set} of $\mathcal{A}$ is a sub-collection $\mathcal{A}' \subseteq \mathcal{A}$ satisfying the following condition: for any $Q \subseteq U$ with $|Q| \leq q$, there exists $A \in \mathcal{A}$ satisfying $A \cap Q = \emptyset$ iff there exists $A' \in \mathcal{A}'$ satisfying $A' \cap Q = \emptyset$.
%If all sets in $\mathcal{A}$ are of size at most $p$, then there exists a $q$-representative set of $\mathcal{A}$ of size $\binom{p+q}{q}$ \cite{fomin2016efficient}.
Let $\mathcal{A}$ be a collection of subgraphs of a graph $G$.
We say $\mathcal{A}' \subseteq \mathcal{A}$ is a \textit{$q$-representative set} of $\mathcal{A}$ if $\{V(A'): A' \in \mathcal{A}'\}$ is a $q$-representative set of $\{V(A): A \in \mathcal{A}\}$.
\begin{lemma}[\cite{fomin2016efficient}] \label{lem-repset}
Let $\mathcal{A}$ be a collection of sets whose sizes are at most $p$.
Then there exists a $q$-representative set $\mathcal{A}' \subseteq \mathcal{A}$ such that $|\mathcal{A}'| \leq \binom{p+q}{q}$.
Furthermore, such a representative set can be computed in $(p+q)^{O(q)} \cdot |\mathcal{A}|$ time.
\end{lemma}

\paragraph{Graph separators and treewidth.}
We say a graph $G$ admits \textit{balanced $(\eta,\mu,\rho)$-separators} if for every induced subgraph $H$ of $G$, there exists $S \subseteq V(H)$ of size at most $\eta \cdot \omega^\mu(H) \cdot |V(H)|^\rho$ such that every connected component of $H - S$ contains at most $\frac{1}{2} |V(H)|$ vertices, where $\omega(H)$ denotes the size of a maximum clique in $H$.
We denote by $\mathcal{G}(\eta,\mu,\rho)$ the class of all graphs admitting balanced $(\eta,\mu,\rho)$-separators.
We only focus on the case $\rho < 1$, since all graphs are contained in $\mathcal{G}(1,0,1)$.

A \textit{tree decomposition} of a graph $G$ is a pair $(T,\beta)$ where $T$ is a tree and $\beta: T \subseteq 2^{V(G)}$ maps each node $t \in T$ to a set $\beta(t) \subseteq V(G)$ called the \textit{bag} of $t$ such that
\textbf{(i)} $\bigcup_{t \in T} \beta(t) = V(G)$, \textbf{(ii)} for any edge $(u,v) \in E(G)$, there exists $t \in T$ with $u,v \in \beta(t)$, and \textbf{(iii)} for any $v \in V(G)$, the nodes $t \in T$ with $v \in \beta(t)$ form a connected subset in $T$.
The \textit{width} of $(T,\beta)$ is $\max_{t \in T} |\beta(t)| - 1$.
The \textit{treewidth} of a graph $G$, denoted by $\mathbf{tw}(G)$, is the minimum width of a tree decomposition of $G$.

\begin{lemma}[\cite{DorakN2016}] \label{lem-separator=tw}
    %Let $\mathcal{G}$ be a graph class admitting $(\eta,\mu,\rho)$-separators.
    Let $\mathcal{G} \subseteq \mathcal{G}(\eta,\mu,\rho)$ where $\eta, \mu \geq 0$ and $\rho < 1$.
    Then for any graph $G \in \mathcal{G}$ of $n$ vertices, we have $\mathbf{tw}(G) \leq \frac{2^\rho \eta \cdot \omega^{\mu}(G)}{2^\rho - 1} \cdot n^\rho$.
\end{lemma}
\begin{proof}
We prove the lemma by induction on $|V(G)|$.
Suppose the statement holds when all $G \in \mathcal{G}$ with $|V(G)| \leq n-1$.
Consider a graph $G \in \mathcal{G}$ with $|V(G)| = n$.
By assumption, there is a balanced separator $S \subseteq V(G)$ of $G$ with $|S| \leq \eta \cdot \omega^{\mu}(G)\cdot n^\rho$.
Let $C_1,\dots,C_r$ be the connected components of $G-S$.
Then $|V(C_i)| \leq \frac{n}{2}$ for all $i \in [r]$.
By our induction hypothesis, 
\begin{equation*}
    \mathbf{tw}(C_i) \leq \frac{2^\rho \eta \cdot \omega^{\mu}(C_i)}{2^\rho - 1} \cdot (\frac{n}{2})^\rho \leq \frac{\eta \cdot \omega^{\mu}(G)}{2^\rho-1} \cdot n^\rho.
\end{equation*}
For $i \in [r]$, let $(T_i,\beta_i)$ be a tree decomposition of $C_i$ such that $|\beta_i(t)| \leq \frac{\eta \cdot \omega^{\mu}(G)}{2^\rho-1} \cdot n^\rho + 1$ for all nodes $t \in T_i$.
For convenience, we view each $T_i$ as a rooted tree by picking an arbitrary node $t_i \in T_i$ as its root.
Let $T$ be a tree consisting of a root node with subtrees $T_1,\dots,T_r$.
For each node $t \in T$, we define $\beta(t) = S$ if $t$ is the root of $T$ and $\beta(t) = \beta_i(t) \cup S$ if $t \in T_i$.
We now verify that $(T,\beta)$ is a tree decomposition of $G$.
For a vertex $v \in S$, the bags of all nodes of $T$ contain $v$.
For a vertex $v \in V(C_i)$, the nodes of $T$ whose bags contain $v$ are exactly those in $T_i$, which are connected in $T$.
Consider an edge $(u,v) \in E(G)$.
If $u,v \in S$, then $u,v \in \beta(t)$ for all $t \in T$.
Assume $u \notin S$ without loss of generality.
Then $u \in V(C_i)$ for some $i \in [r]$.
If $v \in V(C_i)$, then $u,v \in \beta_i(t)$ for some $t \in T_i$ and hence $u,v \in \beta(t)$.
On the other hand, if $v \notin V(C_i)$, then $v \in S$.
Let $t \in T_i$ be a node such that $u \in \beta_i(t)$.
Then $u,v \in \beta(t)$.
Therefore, $(T,\beta)$ is a tree decomposition of $G$.
Furthermore, 
\begin{equation*}
    |\beta(t)| \leq \frac{\eta \cdot \omega^{\mu}(G)}{2^\rho-1} \cdot n^\rho +1 + |S| \leq \frac{2^\rho \eta \cdot \omega^{\mu}(G)}{2^\rho - 1} \cdot n^\rho +1
\end{equation*}
for all $t \in T$.
So we have $\mathbf{tw}(G) \leq \frac{2^\rho \eta \cdot \omega^{\mu}(G)}{2^\rho - 1} \cdot n^\rho$.
\end{proof}


\paragraph{Expansion, admissibility, and weak coloring numbers.}
A graph $H$ is a \textit{depth-$r$ minor} of $G$, denoted by $H \preceq_r G$, if $H$ is a minor of $G$ where each vertex $v \in V(H)$ corresponds to an induced subgraph $G' \subseteq G$ with radius at most $r$ (i.e., $G'$ is contracted to the vertex $v$ in $H$). 
For a graph $G$ and $r \in \mathbb{N}$ be an integer, define $\nabla_r(G) =\sup \{ |E(H)|/|V(H)|: H \preceq_r G\}$.
We say that a graph class $\mathcal{G}$ has \textit{bounded expansion}, if there is a function $f: \mathbb{N}\rightarrow \mathbb{N}$ such that $\nabla_r(G) \leq f(r)$ for all $G \in \mathcal{G}$ and all $r \in \mathbb{N}$.
%We use $\nabla_r(\mathcal{G})$  to denote $\sup_{G\in \mathcal{G}} \nabla_r(G)$. 
If $f$ is a polynomial (resp., single-exponential) function, then $\mathcal{G}$ is a class of \textit{polynomial expansion} (resp., \textit{single-exponential expansion}).
By the result of Dvo\v{r}\'{a}k and Norin~\cite{DorakN2016}, a graph class $\mathcal{G}$ is of polynomial expansion iff $\mathcal{G} \subseteq \mathcal{G}(\eta,0,\rho)$ for some $\eta \geq 0$ and $\rho < 1$.

Let $G$ be a graph and $\sigma$ be an ordering of $V(G)$.
For $r \in \mathbb{N}$, the \textit{$r$-admissibility} of a vertex $v \in V(G)$ in $G$ under $\sigma$, denoted by $\text{adm}_r(G,\sigma,v)$, is equal to one plus the maximum size of a family of paths ${\cal P}$ with the following properties. 
\begin{itemize}
\item Every path in ${\cal P}$ is from $v$ to some vertex smaller than $v$ in $\sigma$ and has length at most $r$. 
\item Paths in ${\cal P}$ are pairwise vertex-disjoint apart from sharing the endpoint $v$.
\end{itemize}
The \textit{$r$-admissibility} of $G$ \textit{under $\sigma$} is defined as $\textnormal{adm}_r(G,\sigma) = \max_{v\in V(G)} \text{adm}_r(G,\sigma,v)$.
Finally, the \textit{$r$-admissibility} of $G$ is defined as $\text{adm}_r(G) = \min_{\sigma \in \Sigma(G)} \textnormal{adm}_r(G,\sigma)$ where where $\Sigma(G)$ is the set of all orderings of $V(G)$.

The \textit{weak coloring numbers} are defined in a similar fashion.
For $u,v \in V(G)$, we write $u <_\sigma v$ if $u$ is before $v$ under the ordering $\sigma$.
The notations $>_\sigma$, $\leq_\sigma$, $\geq_\sigma$ are defined similarly.
For an integer $r \geq 0$, $u$ is \textit{weakly $r$-reachable} from $v$ \textit{under $\sigma$} if there is a path $\pi$ between $v$ and $u$ of length at most $r$ such that $u$ is the largest vertex on $\pi$ under the ordering $\sigma$, i.e., $u \geq_\sigma w$ for all $w \in V(\pi)$.
Let $\text{WR}_r(G,\sigma,v)$ denote the set of vertices in $G$ that are weakly $r$-reachable from $v$ under $\sigma$.
The \textit{weak $r$-coloring number} of $G$ \textit{under $\sigma$} is defined as $\mathsf{wcol}_r(G,\sigma) = \max_{v \in V(G)} |\text{WR}_r(G,\sigma,v)|$.
Finally, the \textit{weak $r$-coloring number} of $G$ is defined as $\mathsf{wcol}_r(G) = \min_{\sigma \in \Sigma(G)} \mathsf{wcol}_r(G,\sigma)$.

\begin{lemma}[\cite{DorakN2016}] \label{lem-edgenumber}
    %Let $\mathcal{G}$ be a graph class admitting $(\eta,0,\rho)$-separators where $\rho < 1$.
    Let $\mathcal{G} \subseteq \mathcal{G}(\eta,0,\rho)$ where $\eta \geq 0$ and $\rho < 1$.
    %Then there exists a constant $c > 0$ only depending on $\rho$ such that 
    For any graph $G \in \mathcal{G}$ of $n$ vertices, $|E(G)| = \eta^{O(1)} \cdot n$ and $G$ is $\eta^{O(1)}$-degenerate.
    The constants hidden in $O(\cdot)$ only depend on $\rho$.
\end{lemma}

\begin{lemma}[\cite{nevsetvril2008grad}] \label{lem-nablawcol}
    %Let $\mathcal{G}$ be a graph class admitting $(\eta,0,\rho)$-separators where $\rho < 1$.
    Let $\mathcal{G} \subseteq \mathcal{G}(\eta,0,\rho)$ where $\eta \geq 0$ and $\rho < 1$.
    %Then there exists a constant $c > 0$ only depending on $\rho$ such that the following conditions hold.
    Then the following conditions hold.
    \begin{enumerate}[(i)]
        \item For any $G \in \mathcal{G}$ and $r \geq 0$, $\nabla_r(G) \leq (\eta r)^{O(1)}$.
        \item For any $G \in \mathcal{G}$ and $r \geq 0$, $\textnormal{wcol}_r(G) \leq (\eta r)^{O(r^2)}$.
    \end{enumerate}
    The constants hidden in $O(\cdot)$ only depend on $\rho$.
\end{lemma}

%\begin{proposition}[\cite{dvorak2011constantfactor}]
%\label{prop:adm:wcol}
%For every $r\in {\mathbb N}$, graph $G$, and its vertex ordering $\sigma$, the following inequalities hold:  
%$\textnormal{adm}_r(G,\sigma)\leq \textnormal{wcol}_r(G,\sigma) \leq 1+r(\textnormal{adm}_r(G,\sigma)-1)^{r^2}$. 
%\end{proposition} 

%\begin{proposition}[Corollary 4.1, Sparsity book]
%    $\widetilde{\nabla}_r(G) \leq \nabla_r(G) $ 
%\end{proposition}

\begin{lemma} \label{lem-ordering}
    Given a graph $G$ of $n$ vertices and $m$ edges, and a number $r \in [n]$, one can compute in $O(n^3 m)$ time an ordering $\sigma$ of $V(G)$ such that $\textnormal{wcol}_r(G,\sigma) \leq (7r \cdot \nabla_r(G))^{3r^2}$.
\end{lemma}
\begin{proof}[Proof sketch]
The lemma follows from \cite{dvorak2011constantfactor}. For completeness, we give a proof sketch here. 
%
For a subset $S\subseteq V(G)$ and $v\in V(G)$, define $b_r(v,S)$ to be the
maximum cardinality of a family ${\cal P}$ of paths in $G$ with the following properties. 

\begin{itemize}
\item Every path in ${\cal P}$ has length at most $r$, and it is from $v$ to some vertex in $S$ with all internal vertices from $V(G)\setminus S$.  
\item Paths in ${\cal P}$ are pairwise vertex-disjoint apart from sharing the endpoint $v$.
\end{itemize}

Let $\sigma'=(v_1,v_2,\ldots,v_n)$ be the ordering defined as follows. Assuming the suffix $v_{i+1},\ldots,v_n$, the vertex $v_i$ is defined as follows. Let $S_i=V(G)\setminus \{v_{i+1},\ldots,v_n\}$. Then, $v_i$ to be a vertex $v$ in $S_i$ that minimizes $b_{r}(v,S_i)$. 
\medskip

\noindent
\textit{Claim 1.}
$\textnormal{adm}_r(G,\sigma')=\textnormal{adm}_r(G)$.
\medskip

\noindent
\textit{Proof.}
For an ordering $\sigma=(v_1,v_2,\ldots,v_n)$ of $V(G)$ and integers $i,j\in [n]$, we write $\sigma[i]=v_i$ and $\sigma[i,j]=(v_i,v_{i+1},\ldots,v_{j})$. 
%For a function $f: D \rightarrow R$ and $X\subseteq D$, $f(X)=\{f(x)~|~x\in D\}$. 
We prove the following statement using induction.
For each $j\in \{0,1,\ldots,n\}$, there is an ordering $\sigma_j$ of $V(G)$ such that $\textnormal{adm}_r(G,\sigma_j)=\textnormal{adm}_r(G)$ and the $j$-length suffix of the ordering $\sigma_j$ is $v_{n-j+1},\ldots,v_n$. The base case is when $j=0$ and the statement is trivially true. Now consider the induction step when $j>0$. By induction hypothesis, we have that there is an ordering $\sigma_{j-1}$ of $V(G)$ such that 
$\textnormal{adm}_r(G,\sigma_{j-1})=\textnormal{adm}_r(G)$ and the $(j-1)$-length suffix of the ordering $\sigma_{j-1}$ is $v_{n-j+2},\ldots,v_n$. Let $i+1=n-j+2$. 
Recall the construction of the ordering $\sigma'$. 
Recall that $S_i=\{v_{i+1},\ldots,v_n\}$. Moreover, for any $y\in S_i$, $b(v_i,S_i)\leq b(y,S_i)$. Next, we construct an ordering $\sigma_j$ from $\sigma_{j-1}$ with the required properties. 
%Let $w$ be the element just before $v_{n-j+2}$ in the ordering $\sigma_{j-1}$. That is, $w$ is the largest element in the ordering $\sigma_{j-1}$ such that $w<v_{n-j+2}$. 
If $\sigma_{j-1}[i]=v_{i}$, then $\sigma_j=\sigma_{j-1}$. It is easy to see that $\sigma_j$ satisfies the required properties in this case. Suppose $\sigma_{j-1}[i]\neq v_{i}$. Then, let $q<i$ be the index such that $\sigma_{j-1}[q]=v_{i}$. We define $\sigma_j$ to be the ordering obtained by deleting $v_{i}$ from $\sigma_{j-1}$ and inserting it just before $v_{i+1}$. That is, if $\sigma_{j-1}[1,i]=(u_1,u_2,\ldots,u_{i})$, then $\sigma_j$ is the ordering $(u_1,\ldots,u_{q-1},u_{q+1},\ldots, u_{i},v_{i},\ldots,v_n)$.  Clearly, the $j$-length suffix of the ordering $\sigma_j$ is $(v_{i},\ldots,v_n)$. 

Next, we prove that $\textnormal{adm}_r(G,\sigma_j)=\textnormal{adm}_r(G)$.
Towards that it is enough to prove that for each $x\in V(G)$, $\textnormal{adm}_r(G,\sigma_j,x) \leq \textnormal{adm}_r(G)$. Fix a vertex $x\in V(G)$ and let $s\in [n]$ be the index such that $\sigma_j[s]=x$.
We distinguish four cases as follows.

\begin{enumerate}
    \item $1\leq s \leq q-1$.
    Since $\textnormal{adm}_r(G,\sigma_{j-1})=\textnormal{adm}_r(G)$ and $\sigma_{j-1}[1,s]=\sigma_j[1,s]$, we get that $\textnormal{adm}_r(G,\sigma_j,x)= \textnormal{adm}_r(G,\sigma_{j-1},x) \leq \textnormal{adm}_r(G)$.
    \item $q\leq s \leq i-1$.
    For the sake of contradiction, assume that $\textnormal{adm}_r(G,\sigma_j,x)>\textnormal{adm}_r(G)$. Let ${\cal P}$ be a family of paths that witnesses the assumption  $\textnormal{adm}_r(G,\sigma_j,x)>\textnormal{adm}_r(G)$. 
Here, $\textnormal{adm}_r(G,\sigma_j,x)=1+|{\cal P}|$. 
Clearly $v_{i}$ should belong to a path in ${\cal P}$. Otherwise the existence of ${\cal P}$ implies that $\textnormal{adm}_r(G,\sigma_{j-1},x)\geq 1+|{\cal P}|$. This will contradicts the assumption that  $\textnormal{adm}_r(G,\sigma_{j-1})=\textnormal{adm}_r(G)$.
Let $P$ be the path in ${\cal P}$ such that $v_{i}\in V(P)$. Let $P'$ be the subpath of $P$ from $x$ to $v_{i}$. Now let ${\cal P}'=({\cal P}\setminus \{P\})\cup \{P'\}$. Notice that ${\cal P}'$ satisfies the conditions in the definition of admissibility for the vertex $x$ and the ordering $\sigma_{j-1}$. This implies that 
$\textnormal{adm}_r(G,\sigma_{j-1},x)\geq 1+|{\cal P}'|=|{\cal P}|$. This is a contradiction.
    \item $s=i$.
    Equivalently, we have $x=v_i$.
    The choice of $v_i$ in the construction of $\sigma'$ implies that  $\textnormal{adm}_r(G,\sigma_j,x) \leq \textnormal{adm}_r(G,\sigma_{j-1},\sigma_{j-1}[i])\leq \textnormal{adm}_r(G)$. 
    \item $n-j+2\leq i \leq n$.
    Since $\textnormal{adm}_r(G,\sigma_{j-1})=\textnormal{adm}_r(G)$ and $\sigma_{j-1}[i,n]=\sigma_j[i,n]$, we get that $\textnormal{adm}_r(G,\sigma_j,x)= \textnormal{adm}_r(G,\sigma_{j-1},x) \leq \textnormal{adm}_r(G)$.
\end{enumerate}
This completes the proof of the claim. 
\hfill $\lhd$
\medskip

Next, we explain how to compute an ordering $\sigma$ in time $O(n^3 m)$ such that $\textnormal{adm}_r(G,\sigma)\leq r \cdot \textnormal{adm}_r(G)$. Assume we have computed the suffix $w_{i+1},\ldots,w_n$ of $\sigma'$. Let $W_i=V(G) \backslash \{w_{i+1},\ldots,w_n\}$. 
%For each $v\in W_i$, let ${\cal P}_v$ be a ma 
Then for each $v\in W_i$, we greedily compute a family ${\cal P}_v$ of paths (as in the definition of $b_r(v,W_i)$). 
Since each path in ${\cal P}_v$ may kill at most $r$ paths 
in any family of such paths, we have that 
 $|{\cal P}_v|\geq \frac{1}{r}\cdot b_r(v,W_i)$. Notice that we can compute ${\cal P}_v$ in $O(nm)$ time for each $v\in W_i$, because each path in ${\cal P}_v$ can be computed in time $O(m)$. We define $w_i$ to the vertex $v$ that minimizes $|{\cal P}_v|$. Similar to the proof that $\sigma'$ is an optimum ordering for $r$-admissibilty, one can prove that  $\textnormal{adm}_r(G,\sigma)\leq r \cdot  \textnormal{adm}_r(G)$. Since there are at most $n^2$ computations of families of paths as explained above, the total running time will be $O(n^3m)$. 
We then show that $\textnormal{wcol}_r(G,\sigma) \leq (7r \cdot \nabla_r(G))^{3r^2}$. 
It was known that $\textnormal{adm}_r(G) \leq 1+6r \left( \nabla_r(G) \right)^3$; see for example Lemma~3.2 in the lecture note on sparsity by Pilipczuk and Pilipczuk\footnote{\url{https://www.mimuw.edu.pl/~mp248287/sparsity2/lectures/chapter2.pdf}}. 
Also, $\text{wcol}_r(G,\sigma) \leq  1+r(\text{adm}_r(G,\sigma)-1)^{r^2}$ by~\cite{dvorak2011constantfactor}.
So we have
\begin{eqnarray*}
\textnormal{wcol}_r(G,\sigma) &\leq&  1+r(\textnormal{adm}_r(G,\sigma)-1)^{r^2}\\
&\leq& 1+r (6r\left( \nabla_r(G) \right)^3)^{r^2} \\
&\leq& (7r \cdot \nabla_r(G))^{3r^2}
\end{eqnarray*}
This completes the proof of the lemma. 
\end{proof}

%For graphs $F$ and $G$, an \textit{$F$-copy} in $G$ is a pair $(H,\pi)$ where $H \subseteq G$ and $\pi: V(H) \rightarrow V(F)$ is an isomorphism between $H$ and $F$.
\paragraph{Augmentations.}
Let $\mathcal{G}$ be a graph class, and $\gamma \geq 0$ be an integer.
The \textit{$\gamma$-augmentation} of $\mathcal{G}$ is another graph class $\mathcal{G}'$ defined as follows.
For every graph $G \in \mathcal{G}'$ and every ordering $\sigma$ of $V(G)$ such that $\text{wcol}_\gamma(G,\sigma) = \text{wcol}_\gamma(G)$, we include in $\mathcal{G}'$ a graph $G'$, which is obtained from $G$ by adding edges $(u,v)$ with $v \in \text{WR}_\gamma(G,\sigma,u)$.
The augmentation has the following property.

\begin{lemma} \label{lem-augmentation}
    %Let $\mathcal{G}$ be a graph class admitting $(\eta,\mu,\rho)$-separators,
    Let $\mathcal{G} \subseteq \mathcal{G}(\eta,\mu,\rho)$ where $\eta, \mu \geq 0$ and $\rho < 1$.
    Also, let $\mathcal{G}'$ be the $\gamma$-augmentation of $\mathcal{G}$.
    Then $\mathcal{G}' \subseteq \mathcal{G}(\eta',\mu,\rho)$ for $\eta' = (\eta \gamma)^{O(\gamma^2)}$.
    The constant hidden in $O(\cdot)$ only depends on $\rho$.
\end{lemma}
\begin{proof}
Let $G' \in \mathcal{G}'$.
By the construction of $\mathcal{G}'$, there exists $G \in \mathcal{G}$ and an ordering $\sigma$ of $V(G)$ satisfying $\text{wcol}_\gamma(G) = \text{wcol}_\gamma(G,\sigma)$ such that $G'$ is obtained from $G$ by adding edges $(u,v)$ with $v \in \text{WR}_\gamma(G,\sigma,u)$.
We have $V(G) = V(G')$.
Set $\eta' = \eta \cdot \text{wcol}_\gamma(G)$.
Thus, $\eta' = (\eta \gamma)^{O(\gamma^2)}$ by Lemma~\ref{lem-nablawcol}.
For any subset $V \subseteq V(G')$, we want to show that $G'[V]$ has a balanced separator of size $\eta' \cdot \omega^\mu(G') \cdot n^{\rho}$, where $n = |V|$.
By assumption $G[V]$ has a balanced separator $S$ of size at most $\eta \cdot \omega^\mu(G) \cdot n^{\rho}$.
Define $S' = \bigcup_{s \in S} (V \cap \text{WR}_\gamma(G,\sigma,s))$.
We claim that $S'$ is a balanced separator of $G'[V]$.
It suffices to show that every connected component of $G'[V] - S'$ is contained in a connected component of $G[V] - S$.
Consider a connected component $C'$ of $G'[V] - S'$.
As $S \subseteq S'$, $V(C') \subseteq V \backslash S' \subseteq V \backslash S$.
Thus, there exists a connected component $C$ of $G[V]-S$ such that $V(C) \cap V(C') \neq \emptyset$.
Assume $V(C') \nsubseteq V(C)$, in order to deduce a contradiction.
Let $u \in V(C) \cap V(C')$ and $v \in V(C') \backslash V(C)$.
Since $u,v \in V(C')$ and $C'$ is connected, there is a path $(v_0,v_1,\dots,v_r)$ in $C'$ with $v_0 = u$ and $v_r = v$.
Define $i \in \{0\} \cup [r]$ as the smallest index such that $v_i \notin V(C)$.
Note that such an index exists because $v_r \notin V(C)$.
Furthermore, $i \geq 1$, as $v_0 \in V(C)$.
So we have $v_{i-1} \in V(C)$.
As $(v_{i-1},v_i) \in E(G')$, we have either $v_{i-1} \in \text{WR}_\gamma(G,\sigma,v_i)$ or $v_i \in \text{WR}_\gamma(G,\sigma,v_{i-1})$.
Thus, there exists a path $\pi$ in $G$ of length at most $\gamma$ between $v_{i-1}$ and $v_i$ on which the largest vertex (under the ordering $\sigma$) is either $v_{i-1}$ or $v_i$.
But $v_{i-1} \in V(C)$ and $v_i \notin V(C)$.
So $\pi$ must contain a vertex $s \in S$.
If $v_{i-1}$ is the largest vertex on $\pi$, then $v_{i-1} \in \text{WR}_\gamma(G,\sigma,s)$, since the sub-path $\pi'$ of $\pi$ between $v_{i-1}$ and $s$ has length at most $\gamma$ and the largest vertex on $\pi'$ is $v_{i-1}$.
Similarly, if $v_i$ is the largest vertex on $\pi$, then $v_i \in \text{WR}_\gamma(G,\sigma,s)$.
In other words, we have either $v_{i-1} \in \text{WR}_\gamma(G,\sigma,s)$ or $v_i \in \text{WR}_\gamma(G,\sigma,s)$, which implies that either $v_{i-1} \in S'$ or $v_i \in S$.
This contradicts the fact that $(v_0,v_1,\dots,v_r)$ is a path in $C'$.
Therefore, $S'$ is a balanced separator of $G'[V]$.
Finally, since $|\text{WR}_\gamma(G,\sigma,s)| \leq \text{wcol}_\gamma(G,\sigma) = \text{wcol}_\gamma(G)$ for all $s \in S$, we have $|S'| \leq \text{wcol}_\gamma(G) \cdot |S| \leq \eta' \cdot \omega^\mu(G) \cdot n^\rho \leq \eta' \cdot \omega^\mu(G') \cdot n^\rho$.
\end{proof}



==> subisom.tex <==
In this section, we present our efficient algorithm for \textsc{Subgraph Isomorphism}.
Our algorithm can be applied to any graphs, and has the desired running time on certain graph classes.

A \textit{subgraph list} of a graph $G$ refers to a collection $\mathcal{S}$ of subgraphs of $G$.
We say a subgraph list $\mathcal{S}$ of $G$ is $t$-\textit{exhaustive} if for any (nonempty) subgraph $H \subseteq G$ with $|V(H)| \leq t$, there exists $H' \in \mathcal{S}$ such that $H' \simeq H$.
To solve \textsc{Subgraph Isomorphism}, we design the following general algorithm for computing a $t$-exhaustive subgraph list of a graph, whose running time depends on the weak coloring number of the graph with respect to a given ordering of the vertices.
Recall that $b_t(G) = |E(H)|/|V(H)|$ where $H$ is the densest $t$-vertex subgraph of $G$.

\sublist*

Note that once we have the $t$-exhaustive subgraph list $\mathcal{S}$ of $G$ in the above theorem, we can directly use it to solve \textsc{Subgraph Isomorphism} on $G$.
Indeed, given a graph $F$ of $t$ vertices, we only need to check every $H \in \mathcal{S}$ and test whether $H \simeq F$.
Using the quasipolynomial-time algorithm for \textsc{Graph Isomorphism} \cite{babai2016graph}, the entire time cost is $2^{\log^{O(1)} t} \cdot |\mathcal{S}| = (2^{b_t(G)}+\textnormal{wcol}_t(G,\sigma))^{O(t)} \cdot n$.

\subsection{The algorithm} \label{sec-subisoalg}

Let $(G,\sigma)$ be the input of the algorithm of Theorem~\ref{thm-sublist}.
For a subset $S \subseteq V(G)$, the notations $\min(S)$ and $\max(S)$ denote the smallest vertex and the largest vertex in $S$ under the ordering $\sigma$.
Before discussing the algorithm, we first define a relation among the subgraphs of a graph $G$.
For a subset $X \subseteq V(G)$ and two subgraphs $H,H' \subseteq G$, we write $H \simeq_X H'$ if there exists an isomorphism $\pi: V(H) \rightarrow V(H')$ between $H$ and $H'$ such that $\pi(x) = x$ for all $x \in V(H) \cap X$ and $\pi^{-1}(x) = x$ for all $x \in V(H') \cap X$.
Clearly, $\simeq_X$ is an equivalent relation among all subgraphs of $G$.
An intuitive view of the relation $\simeq_X$ is the following.
We make $G$ a \textit{labeled} graph by assigning distinct labels to the vertices in $X$ and assigning identical labels (different from the labels for $X$) to the other vertices of $G$.
Then $\simeq_X$ is just the isomorphism relation among the subgraphs of $G$, viewed as labeled graphs.

Our algorithm for computing $t$-exhaustive subgraph lists is presented in Algorithm~\ref{alg-subiso}.
In line~1, we compute $W_v = \text{WR}_t(G,\sigma,v)$ for all $v \in V(G)$.
Note that $|W_v| \leq \textnormal{wcol}_t(G,\sigma)$.
Initially, we include in $\mathcal{S}$ the subgraphs of $G$ which have at most $t$ vertices all contained in some $W_v$ (line~2).
Then the algorithm consists of two phases: the for-loop in line~3-8 and the for-loop in 9-12.
Basically, the first phase constructs the \textit{connected} subgraphs of $G$ (of at most $t$ vertices), while the second phase further constructs the disconnected ones.

The first phase consists of $t$ iterations.
In every iteration, we update the subgraph list $\mathcal{S}$ as follows.
For each vertex $v \in V(G)$, let $\mathcal{S}_v \subseteq \mathcal{S}$ consist of all graphs containing $v$ (line~5).
In line~6, we use a sub-routine \textsc{Rep}.
For a collection $\mathcal{A}$ of subgraphs of $G$, a subset $X \subseteq V(G)$, and an integer $q \in \mathbb{N}$, $\textsc{Rep}(\mathcal{A},X,q)$ computes and returns a sub-collection $\mathcal{R} \subseteq \mathcal{A}$ as follows.
First, it partitions $\mathcal{A}$ into equivalence classes using the equivalence relation $\simeq_X$.
Then for each equivalence class $\mathcal{C} \subseteq \mathcal{A}$, it computes a $q$-representative set of $\mathcal{C}$.
The collection $\mathcal{R}$ is defined as the union of all representative sets, and is returned by the sub-routine.
In the algorithm, we call $\textsc{Rep}(\mathcal{S}_v,W_v,t)$, and let $\mathcal{R}_v \subseteq \mathcal{S}_v$ be the collection returned (line~6).
Then we construct another collection $\mathcal{U}_v$ which consists of all subgraphs of $G$ that can be represented as the union of three graphs in $\mathcal{R}_v$ (line~7).
The collections $\mathcal{R}_v$ and $\mathcal{U}_v$ are constructed for every $v \in V(G)$.
At the end of the iteration, we define the new $\mathcal{S}$ as the union of all $\mathcal{R}_v$ and all $\mathcal{U}_v$.

%We first compute an ordering $\sigma$ of $V(G)$ such that $\text{adm}_r(G,\sigma) \leq r \cdot \text{adm}_r(G)$ for all $r \geq 0$.
%Such an ordering can be computed in $O(n)$ time.
%As $\mathcal{G}$ is of polynomial expansion, $\text{adm}_r(G,\sigma) = r^{O(1)}$ and thus $\text{wcol}_r(G,\sigma) = r^{O(r^2)}$.

%For a vertex $v \in V(G)$ and an integer $r \geq 0$, we write $W_v^r = \text{WR}_r(G,\sigma,v)$ for convenience.
%We first compute the sets $W_v^k$ for all $v \in V(G)$.
%This can be done in $O(\textnormal{wcol}_k(G,\sigma) \cdot (n+m))$ time.

\begin{algorithm}[h]
    \caption{\textsc{Subgraph}$(G,\sigma,k)$}
    \begin{algorithmic}[1]
        %\State $k \leftarrow |V(H)|$
        \State $W_v \leftarrow \text{WR}_t(G,\sigma,v)$ for all $v \in V(G)$
        %\State $\mathcal{X} = \{X \subseteq V(G): |X| \leq k \text{ and } \min(X) \in X \subseteq W_{\min(X)}\}$
        \State $\mathcal{S} \leftarrow \{H \subseteq G: |V(H)| \leq t \text{ and } V(H) \subseteq W_v \text{ for some } v \in V(G)\}$
        \For{$i=1,\dots,t$}
            %\For{all $X \in \mathcal{X}$}
                %\State $\mathcal{S}_X \leftarrow \{F \in \mathcal{S}: X \subseteq V(F)\}$
                %\State $\mathcal{R}_X \leftarrow \textsc{Rep}(\mathcal{S}_X,X,k)$
                %\State $\mathcal{U}_X \leftarrow \{F \cup F': F,F' \in \mathcal{R}_X \text{ and } |V(F \cup F')| \leq k\}$
            %\EndFor
            \For{all $v \in V(G)$}
                \State $\mathcal{S}_v \leftarrow \{H \in \mathcal{S}: v \in V(H)\}$
                \State $\mathcal{R}_v \leftarrow \textsc{Rep}(\mathcal{S}_v,W_v,t)$
                \State $\mathcal{U}_v \leftarrow \{H \cup H' \cup H'': H,H',H'' \in \mathcal{R}_v \text{ and } |V(H \cup H' \cup H'')| \leq t\}$
            \EndFor
            \State $\mathcal{S} \leftarrow \bigcup_{v \in V(G)} (\mathcal{R}_v \cup \mathcal{U}_v)$
        \EndFor
        \For{$i=1,\dots,t-1$}
            \State $\mathcal{R} \leftarrow \textsc{Rep}(\mathcal{S},\emptyset,t)$
            \State $\mathcal{U} \leftarrow \{H \cup H': H,H' \in \mathcal{R} \text{ and } |V(H \cup H')| \leq t\}$
            \State $\mathcal{S} \leftarrow \mathcal{R} \cup \mathcal{U}$
        \EndFor
        \State \textbf{return} $\mathcal{S}$
    \end{algorithmic}
    \label{alg-subiso}
\end{algorithm}

The second phase is similar to the first one, and is in fact simpler.
It has $t-1$ iterations.
In every iteration, we update the subgraph list $\mathcal{S}$ as follows.
First, we call $\textsc{Rep}(\mathcal{S},\emptyset,t)$, and let $\mathcal{R} \subseteq \mathcal{S}$ be the sub-collection returned (line~10).
Then we construct another collection $\mathcal{U}$ which consists of all subgraphs of $G$ that can be represented as the union of two graphs in $\mathcal{R}$ (line~10).
Finally, the new $\mathcal{S}$ is the union of $\mathcal{R}$ and $\mathcal{U}$ (line~11).
After $t-1$ iterations, we return $\mathcal{S}$ (line~13).

\subsection{Analysis} \label{sec-subisoana}
In this section, we prove the correctness of Algorithm~\ref{alg-subiso} and analyze its running time.
We first consider the running time, which is easier.
The computation of $W_v$ for all $v$ can be done in $O(\textnormal{wcol}_t(G,\sigma) \cdot t|E(G)|)$ time by~\cite{lokshtanov2023hitting} (Lemma 4.11).
Since $|E(G)| \leq \textnormal{wcol}_1(G,\sigma) \cdot n \leq \textnormal{wcol}_t(G,\sigma) \cdot n$, the time cost of this step is dominated by the bound in Theorem~\ref{thm-sublist}.
For each $v \in V(G)$, 
\begin{equation*}
    |W_v| = |\text{WR}_t(G,\sigma,v)| \leq \textnormal{wcol}_t(G,\sigma).
\end{equation*}
Thus, the initial size of $\mathcal{S}$ is $(\textnormal{wcol}_t(G,\sigma))^{O(t)} \cdot n$.
It suffices to show that each iteration of the first phase and the second phase can be done in $(2^{b_t(G)} + \textnormal{wcol}_t(G,\sigma))^{O(t)} \cdot n$ time.

\begin{observation} \label{obs-rep}
    $\textsc{Rep}(\mathcal{A},X,q)$ can be implemented in $(2^p+q+|X|)^{O(p)} \cdot |\mathcal{A}|$ time and returns a collection of size $(2^p+q +|X|)^{O(p)}$, where $p = \max_{A \in \mathcal{A}} |V(A)|$.
\end{observation}
\begin{proof}
We first bound the number of equivalence classes $\mathcal{A}$ has for the equivalence relation $\simeq_X$.
Suppose $X = \{v_1,\dots,v_r\}$.
For each graph $A \in \mathcal{A}$, we make it as a labeled graph with labels in $\{0\} \cup [r]$ by assigning to a vertex $v \in V(A)$ the label $i \in [r]$ if $v = v_i$ and the label 0 if $v \notin X$.
Then two graphs in $\mathcal{A}$ belong to the same equivalence class for $\simeq_X$ iff they are isomorphic as labeled graphs.
Note that $|E(A)| \leq b_p(G) \cdot p$ for all $A \in \mathcal{A}$.
Let $\mathcal{G}_{p,r}$ be the collection consisting of all different (up to isomorphism) labeled graphs of at most $p$ vertices and at most $b_p(G) \cdot p$ edges with label set $\{0\} \cup [r]$.
The size of $\mathcal{G}_{p,r}$ is bounded by $r^{O(p)} \cdot 2^{O(b_p(G) \cdot p)}$, so is the number of equivalence classes in $\mathcal{A}$.
To efficiently partition $\mathcal{A}$ into equivalence classes, we can first construct $\mathcal{G}_{p,r}$ in $r^{O(p)} \cdot 2^{O(b_p(G) \cdot p)}$ time.
Each graph in $\mathcal{G}_{p,r}$ corresponds to one equivalence class (possibly empty) in $\mathcal{A}$.
Then for each graph $A \in \mathcal{A}$, we find the unique graph in $\mathcal{G}_{p,r}$ isomorphic to $A$, and assign $A$ to the corresponding equivalence class.
This step takes $r^{O(p)} \cdot 2^{O(b_p(G) \cdot p)} \cdot |\mathcal{A}|$ time in total.
For each equivalence class $\mathcal{C} \subseteq \mathcal{A}$, we can apply Lemma~\ref{lem-repset} to compute a $q$-representative set $\mathcal{C}' \subseteq \mathcal{C}$ in $(p+q)^{O(p)} \cdot |\mathcal{C}|$ time, whose size is at most $\binom{p+q}{p} = (p+q)^{O(p)}$.
The total time cost for computing all representative sets is then $(p+q)^{O(p)} \cdot |\mathcal{A}|$.
As a result, $\textsc{Rep}(\mathcal{A},X,q)$ takes $(2^{b_p(G)}+q+r)^{O(p)} \cdot |\mathcal{A}|$ time and returns a collection of size $(2^{b_p(G)}+q+r)^{O(p)}$.
\end{proof}

The above observation implies that for each vertex $v \in V(G)$, $|\mathcal{R}_v| = (2^{b_t(G)}+\textnormal{wcol}_t(G,\sigma))^{O(t)}$ and thus $|\mathcal{U}_v| = (2^{b_t(G)}+\textnormal{wcol}_t(G,\sigma))^{O(t)}$, where $\mathcal{R}_v$ and $\mathcal{U}_v$ are the collections computed in line~6 and line~7.
It follows that the size of the collection $\mathcal{S}$ is always bounded by $(2^{b_t(G)}+\textnormal{wcol}_t(G,\sigma))^{O(t)} \cdot n$ after every iteration of the first phase.
Since each graph $H \in \mathcal{S}$ contains at most $t$ vertices, we can compute $\mathcal{S}_v$ for all $v \in V(G)$ in $t \cdot |\mathcal{S}|$ time.
Indeed, we only need to consider each $H \subseteq V(G)$, and add $H$ to $\mathcal{S}_v$ for all $v \in V(H)$.
Computing $\mathcal{R}_v$ can be done in $(2^{b_t(G)}+\textnormal{wcol}_t(G,\sigma))^{O(t)} \cdot |\mathcal{S}_v|$ time for a single vertex $v \in V(G)$ by Observation~\ref{obs-rep}.
Thus, computing all $\mathcal{R}_v$ takes $(2^{b_t(G)}+\textnormal{wcol}_t(G,\sigma))^{O(t)} \cdot |\mathcal{S}|$ time, because 
%line~6 can be done in $(2^k+\textnormal{wcol}_k(G,\sigma))^{O(k)} \cdot |\mathcal{S}_v|$ time
\begin{equation*}
    \sum_{v \in V(G)} |\mathcal{S}_v| = \sum_{H \in \mathcal{S}} |V(H)| \leq t \cdot |\mathcal{S}|.
\end{equation*}
Computing $\mathcal{U}_v$ can be done in $(2^{b_t(G)}+\textnormal{wcol}_t(G,\sigma))^{O(t)}$ time for a single vertex $v \in V(G)$, since $|\mathcal{R}_v| = (2^{b_t(G)}+\textnormal{wcol}_t(G,\sigma))^{O(t)}$.
So computing all $\mathcal{U}_v$ takes $(2^{b_t(G)}+\textnormal{wcol}_t(G,\sigma))^{O(t)} \cdot n$ time.
Finally, as $|\mathcal{S}| = (2^{b_t(G)}+\textnormal{wcol}_t(G,\sigma))^{O(t)} \cdot n$, we see that each iteration of the first phase can be done in $(2^{b_t(G)}+\textnormal{wcol}_t(G,\sigma))^{O(t)} \cdot n$ time.
The same analysis also applies to the second phase.
We conclude that the time complexity of Algorithm~\ref{alg-subiso} is $(2^{b_t(G)}+\textnormal{wcol}_t(G,\sigma))^{O(t)} \cdot n$.

Next, we prove the correctness of Algorithm~\ref{alg-subiso}, which is less obvious.
We first introduce some basic notions.
For a subgraph $H \subseteq G$, we define the \textit{separating set} of $H$ as follows.
Suppose $V(H) = \{v_1,\dots,v_r\}$ where $v_1 \leq_\sigma \cdots \leq_\sigma v_r$.
Let $i \in [r]$ be the largest index such that $H[\{v_1,\dots,v_i\}]$ is \textit{not} connected (set $i = 0$ if such an index does not exist).
Then the \textit{separating set} of $H$ is simply defined as $\mathsf{sep}(H) = \{v_{i+1},\dots,v_r\}$, which is a subset of $V(H)$.

\begin{fact} \label{fact-sepinX}
    For any connected subgraph $H \subseteq G$ with $|V(H)| \leq t$, we have $\mathsf{sep}(H) \subseteq W_{\min(\mathsf{sep}(H))}$.
\end{fact}
\begin{proof}
Suppose $V(H) = \{v_1,\dots,v_r\}$ where $r \leq t$ and $v_1 \leq_\sigma \cdots \leq_\sigma v_r$.
Let $\mathsf{sep}(H) = \{v_{i+1},\dots,v_r\}$ be the separating set of $H$.
As $H$ is connected, we have $i < r$ and thus $\mathsf{sep}(H) \neq \emptyset$.
Set $v = v_{i+1} = \min(\mathsf{sep}(H))$.
To show $\mathsf{sep}(H) \subseteq W_v$, we want $v_j \in W_v$ for all $j \in \{i+1,\dots,r\}$.
Fix an index $j \in \{i+1,\dots,r\}$.
As $j > i$, by the definition of separating sets, $H[\{v_1,\dots,v_j\}]$ is connected.
So there exists a simple path $\pi$ in $H[\{v_1,\dots,v_j\}]$ between $v$ and $v_j$.
Note that the largest vertex on $\pi$ is $v_j$, and the length of $\pi$ is at most $j$ (and thus at most $t$).
Therefore, $v_j \in \text{WR}_t(G,\sigma,v) = W_v$.
\end{proof}

\begin{lemma} \label{lem-decomp}
    For any connected subgraph $H \subseteq G$ such that $|V(H)| \leq t$ and $\mathsf{sep}(H) \subsetneq V(H)$, there exist $A,B \subsetneq V(H)$ satisfying the following conditions.
    \begin{enumerate}[(i)]
        \item $\min(\mathsf{sep}(H)) \in A \cap B \subseteq \mathsf{sep}(H)$.
        \item $H = H[\mathsf{sep}(H)] \cup H[A] \cup H[B]$.
        \item $H[A]$ and $H[B]$ are connected.        
        \item $A \cap \mathsf{sep}(H) \subseteq \mathsf{sep}(H[A])$ and $B \cap \mathsf{sep}(H) \subseteq \mathsf{sep}(H[B])$.
    \end{enumerate}
\end{lemma}
\begin{proof}
Set $X = \mathsf{sep}(H)$.
Since $X \subsetneq V(H)$, $H-X$ is not connected.
Let $C_1,\dots,C_r$ be the connected components of $H-X$, where $r \geq 2$.
For an index set $I \subseteq [r]$, Define $V_I = N_H[\bigcup_{i \in I} V(C_i)]$ and $H_I = H[V_I]$.
Define $A = V_{\{1\}}$ and $B = V_{\{2,\dots,r\}}$.
Note that $A,B \subsetneq V(H)$, since $A$ does not contain the vertices of $C_2$ and $B$ does not contain the vertices of $C_1$.
We now verify that $A$ and $B$ satisfy the four conditions.
Note that $A \subseteq V(C_1) \cup X$ and $B \subseteq (\bigcup_{i=2}^r V(C_i)) \cup X$.
As $C_1,\dots,C_r$ are disjoint, we have $A \cap B \subseteq \mathsf{sep}(H)$.
To see $\min(X) \in A \cap B$, set $v = \min(X)$.
%Then $X \subseteq W_v$ by Fact~\ref{fact-sepinX}.
\medskip

\noindent
\textit{Claim 1.}
For every $i \in [r]$, $C_i$ is neighboring to $v$ in $H$.
\medskip

\noindent
\textit{Proof.}
By the definition of separating sets, $H - (X \backslash \{v\})$ is connected.
The graph $H - X$ can be obtained from $H - (X \backslash \{v\})$ by removing the vertex $v$.
Thus, every connected component $C_i$ of $H - X$ is neighboring to $v$ in $H - (X \backslash \{v\})$ and thus in $H$.
\hfill $\lhd$
\medskip

Claim~1 directly implies $v \in A \cap B$.
This proves condition (i).
To see condition (ii), first notice that $V(H) = X \cup A \cup B$.
Consider an edge $(u,v) \in E(H)$.
If $u,v \in X$, then $(u,v) \in E(H[X])$.
Otherwise, assume $u \in V(C_i)$ without loss of generality.
Then we have $(u,v) \in E(H[A])$ if $i = 1$ and $(u,v) \in E(H[B])$ if $i \in \{2,\dots,r\}$.
Thus, $H = H[X] \cup H[A] \cup H[B]$.
Next, we verify conditions (iii) and (iv).
This is more complicated than the first two conditions.
\medskip

\noindent
\textit{Claim 2.}
For every nonempty $I \subseteq [r]$ and $X' \subseteq V_I \cap (X \backslash \{v\})$, the graph $H_I - X'$ is connected.
\medskip

\noindent
\textit{Proof.}
Each $C_i$ for $i \in I$ is neighboring to $v$ by Claim~1, which implies $v \in V_I \cap X$.
As $v \notin X'$, we further have $v \in (V_I \cap X) \backslash X'$.
Observe that $H_I - X'$ consists of subgraphs $C_i$ for $i \in I$ and the vertices in $(V_I \cap X) \backslash X'$.
Now each $C_i$ is connected and is neighboring to $v \in (V_I \cap X) \backslash X'$.
%So the subgraph of $F_J - X'$ induced by the vertex set $(\bigcup_{i \in I} C_i) \cup \{v\}$ is connected.
Furthermore, each vertex in $(V_I \cap X) \backslash X'$ is neighboring to $C_i$ for some $i \in I$, by the construction of $V_I$.
Therefore, $H_I - X'$ is connected.
\hfill $\lhd$
\medskip

Claim~2 implies condition (iii).
Indeed, applying Claim~2 with $I = \{1\}$ (resp., $I = \{2,\dots,r\}$) and $X' = \emptyset$ shows that $H[A]$ (resp., $H[B]$) is connected.
Finally, we consider condition (iv).
\medskip

\noindent
\textit{Claim 3.}
For every nonempty $I \subseteq [r]$, $V_I \cap X \subseteq \mathsf{sep}(H_I)$.
\medskip

\noindent
\textit{Proof.}
Set $v' = \min(\mathsf{sep}(H_I))$.
By the definition of separating set, $\mathsf{sep}(H_I) = \{u \in V_I: u \geq_\sigma v'\}$.
Since $X = \mathsf{sep}(H)$, the vertices in $X$ are larger than the vertices of $H-X$ under the ordering $\sigma$.
In particular, the vertices in $V_I \cap X$ are larger than the vertices of $H_I - (V_I \cap X) = \bigcup_{i \in I} C_i$ under $\sigma$.
Therefore, we have either $\mathsf{sep}(H_I) \subsetneq V_I \cap X$ or $V_I \cap X \subseteq \mathsf{sep}(H_I)$.
We observe that the former is not true, and thus we must have $V_I \cap X \subseteq \mathsf{sep}(H_I)$.
Note that $v = \min(V_I \cap X)$, because $v \in V_I \cap X$ by Claim~1 and $v = \min(X)$.
If $\mathsf{sep}(H_I) \subsetneq V_I \cap X$, then $v' >_\sigma v$ and thus $\mathsf{sep}(H_I) \subseteq V_I \cap (X \backslash \{v\})$.
Then Claim~2 implies that $H_I - \mathsf{sep}(H_I)$ is connected.
The only case in which this can happen is when $\mathsf{sep}(H_I) = V(H_I)$.
But this is not true since $v \in V(H_I)$ but $v \notin \mathsf{sep}(H_I)$.
\hfill $\lhd$
\medskip

Note that Claim~3 directly implies condition (iv).
Indeed, $A = V_{\{1\}}$ and $H[A] = H_{\{1\}}$.
Applying Claim~3 with $I = \{1\}$ implies $A \cap X \subseteq \mathsf{sep}(H[A])$.
Similarly, $B = V_{\{2,\dots,r\}}$ and $H[B] = H_{\{2,\dots,r\}}$.
Applying Claim~3 with $I = \{2,\dots,r\}$ implies $B \cap X \subseteq \mathsf{sep}(H[B])$.
\end{proof}

With the notion of separating sets and their properties in hand, we are now ready to prove the correctness of Algorithm~\ref{alg-subiso}.
Our goal is to show that the collection $\mathcal{S}$ returned by Algorithm~\ref{alg-subiso} is $t$-exhaustive.
For $i \in [t]$, we denote by $\mathcal{S}^{(i)}$ the set $\mathcal{S}$ after the $i$-th iteration of the first phase of Algorithm~\ref{alg-subiso}.
For convenience, also let $\mathcal{S}^{(0)}$ be the set $\mathcal{S}$ created in line~2 of Algorithm~\ref{alg-subiso}.

\begin{observation} \label{obs-fullsep}
    $\mathcal{S}^{(0)} \subseteq \mathcal{S}^{(i)}$ for all $i \in [t]$.
    %For any subgraph $H \subseteq G$ such that $|V(H)| \leq k$ and $V(H) \subseteq W_{\min(V(H))}$, we have $H \in \mathcal{S}^{(i)}$ for every $i \in \{0\} \cup [t]$.
\end{observation}
\begin{proof}
Let $H \in \mathcal{S}^{(0)}$.
Then $|V(H)| \leq t$ and $V(H) \subseteq W_v$ for some $v \in V(G)$.
To show $H \in \mathcal{S}^{(i)}$, we apply induction on $i$.
%Clearly, we have $H \in \mathcal{S}^{(0)}$.
Suppose $H \in \mathcal{S}^{(i-1)}$ and we want to show $H \in \mathcal{S}^{(i)}$.
Set $v = \min(V(H))$.
Consider the sets $\mathcal{S}_v$ and $\mathcal{R}_v$ constructed in the $i$-th iteration.
We have $H \in \mathcal{S}_v$.
To show $H \in \mathcal{S}^{(i)}$, it suffices to show $H \in \mathcal{R}_v$, because $\mathcal{R}_v \subseteq \mathcal{S}^{(i)}$.
Since $V(H) \subseteq W_v$, the only subgraph of $G$ having the relation $\simeq_{W_v}$ with $H$ is $H$ itself.
Therefore, one equivalence class of $\mathcal{S}_v$ under $\simeq_{W_v}$ is $\{H\}$.
As $\textsc{Rep}(\mathcal{S}_v,W_v,t)$ contains a $t$-representative set of this equivalence class, we must have $H \in \textsc{Rep}(\mathcal{S}_v,W_v,t)$, i.e., $H \in \mathcal{R}_v$.
It follows that $H \in \mathcal{S}^{(i)}$.
\end{proof}

\begin{observation} \label{obs-firstfor}
    The following statement holds for every $i \in \{0\} \cup [t]$.
    For any (nonempty) connected subgraph $H \subseteq G$ with $|V(H)| \leq i$ and any $Z \subseteq V(G)$ satisfying $|Z|+|V(H)| \leq t$ and $V(H) \cap Z = \emptyset$, there exists $H' \in \mathcal{S}^{(i)}$ such that $H' \simeq_{\mathsf{sep}(H)} H$ and $V(H') \cap Z = \emptyset$.
\end{observation}
\begin{proof}
We prove the statement by induction on $i$.
When $i = 0$, the statement trivially holds.
Suppose it holds for $i-1$, and we show it also holds for $i$.
Consider a connected subgraph $H \subseteq G$ with $|V(H)| \leq i$ and a set $Z \subseteq V(G)$ satisfying $|Z|+|V(H)| \leq t$ and $V(H) \cap Z = \emptyset$.
Set $X = \mathsf{sep}(H)$ and $v = \min(X)$.
Then $X \subseteq W_v$ by Fact~\ref{fact-sepinX}.
If $X = V(H)$, then $V(H) \subseteq W_v = W_{\min(V(H))}$ and thus $H \in \mathcal{S}^{(i)}$ by Observation~\ref{obs-fullsep}.
So assume $X \subsetneq V(H)$.
For convenience, in what follows, the notations $\mathcal{S}_v$, $\mathcal{R}_v$, $\mathcal{U}_v$ denote specifically the corresponding sets constructed in the $i$-th iteration of the first for-loop of Algorithm~\ref{alg-subiso}.
Observe that $H[X] \in \mathcal{R}_v$.
Indeed, $H[X] \in \mathcal{S}^{(i-1)}$ by Observation~\ref{obs-fullsep}, because $X \subseteq W_v = W_{\min(X)}$.
Thus, $H[X] \in \mathcal{S}_v$, as $v \in X$.
Since $X \subseteq W_v$, the only subgraph of $G$ having the relation $\simeq_{W_v}$ with $H[X]$ is $H[X]$ itself.
Thus, one equivalence class of $\mathcal{S}_v$ under $\simeq_{W_v}$ is $\{H[X]\}$.
As $\mathcal{R}_v$ contains a $t$-representative set of this equivalence class, $H[X] \in \mathcal{R}_v$.

By Lemma~\ref{lem-decomp}, there exist $A,B \subsetneq V(H)$ satisfying the conditions in the lemma.
As $A,B \subsetneq V(H)$, we have $|A| \leq i-1$ and $|B| \leq i-1$.
Furthermore, by condition (iii) of Lemma~\ref{lem-decomp}, $H[A]$ and $H[B]$ are connected.
Set $Z_1 = (Z \cup V(H)) \backslash A$.
Clearly, $A \cap Z_1 = \emptyset$.
Furthermore, as $A \subseteq Z \cup V(H)$,
\begin{equation*}
    |Z_1|+|A| = |Z \cup V(H)| = |Z| + |V(H)| \leq t.
\end{equation*}
So by our induction hypothesis, there exists $H_A \in \mathcal{S}^{(i-1)}$ such that $H_A \simeq_{\mathsf{sep}(H[A])} H[A]$ and $V(H_A) \cap Z_1 = \emptyset$.
By condition (i) of Lemma~\ref{lem-decomp}, $v \in A \cap B \subseteq X$, which implies $v \in A \cap X$.
By condition (iv) of Lemma~\ref{lem-decomp}, $A \cap X \subseteq \mathsf{sep}(H[A])$.
So $v \in \mathsf{sep}(H[A])$.
Since $H_A \simeq_{\mathsf{sep}(H[A])} H[A]$ and $\mathsf{sep}(H[A]) \subseteq A$, we have $\mathsf{sep}(H[A]) \subseteq V(H_A)$.
In particular, $v \in V(H_A)$.
This implies $H_A \in \mathcal{S}_v$.
By the construction of $\mathcal{R}_v$, there exists $H_A' \in \mathcal{R}_v$ such that $H_A' \simeq_{W_v} H_A$ and $V(H_A') \cap Z_1 = \emptyset$, because $|Z_1| \leq t$ and $\mathcal{R}_v$ contains a $t$-representative set of the equivalence class of $\mathcal{S}_v$ under $\simeq_{W_v}$ that contains $H_A$.
Note that $|A| = |V(H_A)| = |V(H_A')|$.
Since $A \cap Z_1 = \emptyset$ and $V(H_A') \cap Z_1 = \emptyset$, we have
\begin{equation*}
    |Z_1 \cup V(H_A')| = |Z_1| + |V(H_A')| = |Z_1|+|A| \leq t.
\end{equation*}
%Since $A \cap X \subseteq \mathsf{sep}(H[A]) \subseteq V(H_A)$ and $A \cap X \subseteq X \subseteq W_v$, we have $A \cap X \subseteq V(H_A')$ by the fact that $H_A' \simeq_{W_v} H_A$.
%Again by condition (i) of Lemma~\ref{lem-decomp}, $A \cap B \subseteq A \cap X \subseteq V(H_A')$.

Next, set $Z_2 = (Z_1 \cup V(H_A')) \backslash B$.
Clearly, $B \cap Z_2 = \emptyset$.
We claim $|Z_2| + |B| \leq t$.
Indeed, we have $|Z_2| + |B| = |Z_2 \cup B| = |Z_1 \cup V(H_A') \cup B|$, as $Z_2 \cup B = Z_1 \cup V(H_A') \cup B$.
Observe that $B \subseteq Z_1 \cup V(H_A')$, because $B \backslash A \subseteq Z_1$ and $B \cap A \subseteq V(H_A')$ as shown above.
Thus, $Z_1 \cup V(H_A') \cup B = Z_1 \cup V(H_A')$, which implies $|Z_2| + |B| = |Z_1 \cup V(H_A')| \leq t$.
By our induction hypothesis, there exists $H_B \in \mathcal{S}^{(i-1)}$ such that $H_B \simeq_{\mathsf{sep}(H[B])} H[B]$ and $V(H_B) \cap Z_2 = \emptyset$.
Using the same argument as above, we can further show that there exists $H_B' \in \mathcal{R}_v$ such that $H_B' \simeq_{W_v} H_B$ and $V(H_B') \cap Z_2 = \emptyset$.
We observe the following facts about $H_A'$ and $H_B'$.
\medskip

\noindent
\textit{Claim 1.}
$H_A' \simeq_X H[A]$ and $H_B' \simeq_X H[B]$.
\medskip

\noindent
\textit{Proof.}
We only show $H_A' \simeq_X H[A]$, and the relation $H_B' \simeq_X H[B]$ can be proved in the same way.
We have $H_A' \simeq_X H_A$, because $H_A' \simeq_{W_v} H_A$ and $X \subseteq W_v$.
So it suffices to show $H_A \simeq_X H[A]$.
As $A \cap X \subseteq \mathsf{sep}(H[A])$ and $H_A \simeq_{\mathsf{sep}(H[A])} H[A]$, we have $H_A \simeq_{A \cap X} H[A]$.
On the other hand, we also have $H_A \simeq_{X \backslash A} H[A]$, because $X \backslash A \subseteq Z_1$ and $Z_1$ is disjoint from both $A$ and $V(H_A)$.
Therefore, $H_A \simeq_X H[A]$ and $H_A' \simeq_X H[A]$.
\hfill $\lhd$
\medskip

\noindent
\textit{Claim 2.}
$V(H_A') \cap V(H_B') \subseteq X$.
\medskip

\noindent
\textit{Proof.}
By the construction of $H_B'$, $V(H_B') \cap Z_2 = \emptyset$, i.e., $V(H_B') \cap ((Z_1 \cup V(H_A')) \backslash B) = \emptyset$.
Thus, $V(H_B') \cap (V(H_A') \backslash B) = \emptyset$ and $V(H_A') \cap V(H_B') \subseteq V(H_A') \cap B$.
It suffices to show $V(H_A') \cap B \subseteq X$.
Note that $V(H_A') \cap Z_1 = \emptyset$, i.e., $V(H_A') \cap ((Z \cup V(H)) \backslash A) = \emptyset$.
Thus, $V(H_A') \cap (V(H) \backslash A) = \emptyset$, which implies $V(H_A') \cap (B \backslash A) = \emptyset$ and hence $V(H_A') \cap B \subseteq B \cap A$.
As $A \cap B \subseteq X$, we have $V(H_A') \cap B \subseteq X$, which implies $V(H_A') \cap V(H_B') \subseteq X$.
\hfill $\lhd$
\medskip

We now have $H[X],H_A',H_B' \in \mathcal{R}_v$.
Set $H' = H[X] \cup H_A' \cup H_B'$.
Note that $H' \in \mathcal{U}_v$ and thus $H' \in \mathcal{S}^{(i)}$.
Finally, it suffices to prove that $H' \simeq_X H$.
By Claim~1, there exist bijective maps $\pi_A: V(H_A') \rightarrow A$ and $\pi_B: V(H_B') \rightarrow B$ satisfying the following.
\begin{itemize}
    \item $\pi_A$ (resp., $\pi_B$) is an isomorphism between $H_A'$ and $H[A]$ (resp., $H_B'$ and $H[B]$).
    \item $\pi_A(x) = x$ for all $x \in V(H_A') \cap X$ and $\pi_A^{-1}(x) = x$ for all $x \in A \cap X$.
    \item $\pi_B(x) = x$ for all $x \in V(H_B') \cap X$ and $\pi_B^{-1}(x) = x$ for all $x \in B \cap X$.
\end{itemize}
We then define a map $\pi: V(H') \rightarrow V(H)$ by setting
\begin{equation*}
    \pi(x) = \left\{
    \begin{array}{ll}
        x & \text{if } x \in X, \\
        \pi_A(x) & \text{if } x \in V(H_A'), \\
        \pi_B(x) & \text{if } x \in V(H_B').
    \end{array}
    \right.
\end{equation*}
Claim~2 together with the properties of $\pi_A$ and $\pi_B$ guarantees that $\pi$ is well-defined.
Also, $\pi$ is bijective, as we can easily construct its inverse $\pi^{-1}: V(H) \rightarrow V(H')$ as
\begin{equation*}
    \pi^{-1}(x) = \left\{
    \begin{array}{ll}
        x & \text{if } x \in X, \\
        \pi_A^{-1}(x) & \text{if } x \in A, \\
        \pi_B^{-1}(x) & \text{if } x \in B.
    \end{array}
    \right.
\end{equation*}
The fact $A \cap B \subseteq X$ together with the properties of $\pi_A$ and $\pi_B$ guarantees that $\pi^{-1}$ is well-defined.
We further show that $\pi$ is an isomorphism between $H'$ and $H$, which directly implies $H' \simeq_X H$ because $\pi$ is the identity map when restricted to $X$.
By construction, $H' = H[X] \cup H_A' \cup H_B'$.
On the other hand, $H = H[X] \cup H[A] \cup H[B]$.
Note that $\pi_{|X}$ is the identity map on $X$ and thus is an isomorphism between $H[X]$ and $H[X]$.
Furthermore, $\pi_{|V(H_A')}$ (resp., $\pi_{|V(H_B')}$) is an isomorphism between $H_A'$ (resp., $H_B'$) and $H[A]$ (resp., $H[B]$).
Therefore, by Lemma~\ref{lem-isom}, $\pi$ is an isomorphism between $H'$ and $H$, which implies $H' \simeq_X H$.
\end{proof}

%\begin{corollary} \label{cor-connected}
    %After the first for-loop of Algorithm~\ref{alg-subiso}, the set $\mathcal{S}$ satisfies the following property.
    %For any (nonempty) connected subgraph $F \subseteq G$ and any $Z \subseteq V(G)$ satisfying $|Z|+|V(F)| \leq k$ and $V(F) \cap Z = \emptyset$, there exists $H \in \mathcal{S}$ such that $H \simeq F$ and $V(H) \cap Z = \emptyset$.
%\end{corollary}

Next, we consider the second phase of Algorithm~\ref{alg-subiso}.
For convenience, now we use $\mathcal{S}^{(i)}$, for $i \in [t-1]$, to denote the set $\mathcal{S}$ after the $i$-th iteration of the second phase of Algorithm~\ref{alg-subiso}.
Again, $\mathcal{S}^{(0)}$ denotes the set $\mathcal{S}$ just after the first phase.
\begin{observation}
    The following statement holds for every $i \in [t]$.
    For any (nonempty) subgraph $H \subseteq G$ with at most $i$ connected components and any $Z \subseteq V(G)$ satisfying $|Z|+|V(H)| \leq t$ and $V(H) \cap Z = \emptyset$, there exists $H' \in \mathcal{S}^{(i-1)}$ such that $H' \simeq H$ and $V(H') \cap Z = \emptyset$.
\end{observation}
\begin{proof}
As we did in the proof of Observation~\ref{obs-firstfor}, we apply induction on $i$.
When $i = 1$, the statement is implied by Observation~\ref{obs-firstfor}.
Suppose the statement holds for $i-1$, and we show it also holds for $i$.
Consider a subgraph $H \subseteq G$ with connected components $C_1,\dots,C_r$ (for $r \leq i$) and $Z \subseteq V(G)$ satisfying $|Z|+|V(H)| \leq t$ and $V(H) \cap Z = \emptyset$.
Set $Z_1 = Z \cup (\bigcup_{i=2}^r V(C_i))$.
We have $|Z_1| + |V(C_1)| = |Z| + |V(H)| \leq t$ and $V(C_1) \cap Z = \emptyset$.
So by our induction hypothesis, there exists $H_1 \in \mathcal{S}^{(i-2)}$ such that $H_1 \simeq C_1$ and $V(H_1) \cap Z_1 = \emptyset$.
Then the set $\mathcal{R}$ constructed in line~10 in the $i$-th iteration of the for-loop must contain some $H_1' \subseteq G$ such that $H_1' \sim H_1$ and $V(H_1') \cap Z_1 = \emptyset$.
Next, set $Z_2 = Z \cup V(H_1')$.
We have
\begin{equation*}
    |Z_2| + \left|V\left(\bigcup_{i=2}^r C_i\right)\right| = |Z_1| + |V(H_1')| = |Z_1| + |V(C_1)| \leq t
\end{equation*}
and $V(\bigcup_{i=2}^r C_i) \cap Z_2 = (V(\bigcup_{i=2}^r C_i) \cap Z) \cup (V(\bigcup_{i=2}^r C_i) \cap V(H_1')) = \emptyset$.
As $\bigcup_{i=2}^r C_i$ contains $r-1 \leq i-1$ connected components, by our induction hypothesis, there exists $H_2 \in \mathcal{S}^{(i-2)}$ such that $H_2 \simeq \bigcup_{i=2}^r C_i$ and $V(H_2) \cap Z_2 = \emptyset$.
Also, the set $\mathcal{R}$ constructed in the $i$-th iteration must contain some $H_2' \subseteq G$ such that $H_2' \sim H_2$ and $V(H_2') \cap Z_2 = \emptyset$.
Finally, define $H' = H_1' \cup H_2'$.
Since $H_1',H_2' \in \mathcal{R}$, the set $\mathcal{U}$ constructed in line~11 in the $i$-th iteration of the for-loop contains $H'$, which implies $H' \in \mathcal{S}^{(i-1)}$.
It suffices to show $H' \simeq H$ and $V(H') \cap Z = \emptyset$.
Note that $V(H_1') \cap V(H_2') = \emptyset$, as $V(H_1') \subseteq Z_2$ and $V(H_2') \cap Z_2 = \emptyset$.
It follows that $H' \simeq H$, since $H_1' \simeq H_1 \simeq C_1$ and $H_2' \simeq H_2 \simeq \bigcup_{i=2}^r C_i$.
Furthermore, we also have $V(H') \cap Z = \emptyset$, because $V(H_1') \cap Z \subseteq V(H_1') \cap Z_1 = \emptyset$ and $V(H_2') \cap Z \subseteq V(H_2') \cap Z_2 = \emptyset$.
%This completes the induction argument.
\end{proof}

Note that a graph of $t$ vertices has at most $t$ connected components.
Thus, applying the above observation with $i=t$, we see that the collection $\mathcal{S}$ returned by Algorithm~\ref{alg-subiso} is $t$-exhaustive.
As a result, Algorithm~\ref{alg-subiso} computes a $t$-exhaustive subgraph list of $G$ in $(2^{b_t(G)}+\text{wcol}_t(G,\sigma))^{O(t)} \cdot n$ time.

\subsection{Applications}

As discussed before Section~\ref{sec-subisoalg}, the algorithm of Theorem~\ref{thm-sublist} can be used to solve \textsc{Subgraph Isomorphism} efficiently, as long as the graph has a small weak coloring number and a good ordering $\sigma$ is provided.
Combining it with Lemma~\ref{lem-ordering}, we prove the following corollaries.

\begin{corollary} \label{cor-subisopolyexp}
    %Let $\mathcal{G}$ be a graph class admitting $(\eta,0,\rho)$-separators where $\rho < 1$.
    Let $\mathcal{G} \subseteq \mathcal{G}(\eta,0,\rho)$ where $\eta \geq 0$ and $\rho < 1$.
    Then \textsc{Subgraph Isomorphism} on $\mathcal{G}$ can be solved in $(\eta t)^{O(t^3)} \cdot n + \eta^{O(1)} \cdot n^4$ time.
    The constants hidden in $O(\cdot)$ only depend on $\rho$. 
\end{corollary}
\begin{proof}
In this proof, all $O(\cdot)$ hides constants only depending on $\rho$.
Let $(G,F)$ be an instance of \textsc{Subgraph Isomorphism} where $G \in \mathcal{G}$, $|V(G)| = n$, and $|V(F)| = t$.
By Lemma~\ref{lem-edgenumber}, $|E(G)| = \eta^{O(1)} \cdot n$.
Thus, we can apply Lemma~\ref{lem-ordering} to compute in $\eta^{O(1)} \cdot n^4$ time an ordering $\sigma$ of $V(G)$ such that $\text{wcol}_t(G,\sigma) = (t \cdot \nabla_t(G))^{O(t^2)}$.
By Lemma~\ref{lem-nablawcol}, $\nabla_t(G) = (\eta t)^{O(1)}$ and thus $\text{wcol}_t(G,\sigma) = (\eta t)^{O(t^2)}$.
Now we apply Theorem~\ref{thm-subtwbranch} to solve the instance $(G,F)$ in $(2^{b_t(G)}+\text{wcol}_t(G,\sigma))^{O(t)} \cdot n$ time, i.e., $(\eta t)^{O(t^3)} \cdot n$ time.
The overall running time is then $(\eta t)^{O(t^3)} \cdot n + \eta^{O(1)} \cdot n^4$.
\end{proof}

\begin{corollary} \label{cor-subisoclique}
    %Let $\mathcal{G}$ be a graph class admitting $(\eta,\mu,\rho)$-separators where $\rho < 1$.
    Let $\mathcal{G} \subseteq \mathcal{G}(\eta,\mu,\rho)$ where $\eta, \mu \geq 0$ and $\rho < 1$.
    Then \textsc{Subgraph Isomorphism} on $\mathcal{G}$ can be solved in $t^{O(t^3)} \cdot n + t^{O(1)} \cdot n^4$ time.
    %Here the constants hidden in $O(\cdot)$ only depend on $\eta$, $\mu$, and $\rho$.
\end{corollary}
\begin{proof}
Let $(G,F)$ be an instance of \textsc{Subgraph Isomorphism} where $G \in \mathcal{G}$, $|V(G)| = n$, and $|V(F)| = t$.
Suppose $V(G) = \{v_1,\dots,v_n\}$ and define $G_i = G[\{v_1,\dots,v_i\}]$ for $i \in [n]$.
Set $\eta_0 = \eta t^\mu$.
We first find the smallest index $i \in [n]$ such that $G_i$ is \textit{not} $\eta_0^c$-degenerate, where $c>0$ is the constant in Lemma~\ref{lem-edgenumber} depending on $\rho$.
Testing the degeneracy of a graph can be done in linear time using the algorithm of Matula and Beck \cite{matula1983smallest}.
Thus, this step takes $O(n^3)$ time.
If such an index $i$ does not exist, then $G = G_n$ is $\eta_0^c$-degenerate.
In this case, $\omega(G) \leq \eta_0^c+1$ and thus $G$ admits $(\eta(\eta_0^c+1)^\mu,0,\rho)$-separators.
Applying the algorithm of Corollary~\ref{cor-subisopolyexp}, we can solve the instance $(G,F)$ in $t^{O(t^3)} \cdot n + t^{O(1)} \cdot n^4$ time, because $\eta(\eta_0^c+1)^\mu = t^{O(1)}$.
Assume $i$ exists.
By Lemma~\ref{lem-edgenumber}, $G_i$ does not admit $(\eta_0,0,\rho)$-separators, which implies that $\omega(G_i) > t$.
Therefore, $G_i$ contains a subgraph isomorphic to $F$ and it suffices to solve the instance $(G_i,F)$.
On the other hand, $G_{i-1}$ is not $\eta_0^c$-degenerate and hence $\omega(G_{i-1}) \leq \eta_0^c+1$, which implies $\omega(G_i) \leq \eta_0^c+2$ and $G_i$ admits $(\eta(\eta_0^c+2)^\mu,0,\rho)$-separators.
Again, applying the algorithm of Corollary~\ref{cor-subisopolyexp}, we can solve $(G_i,F)$ in $t^{O(t^3)} \cdot n + t^{O(1)} \cdot n^4$ time.
\end{proof}

\begin{corollary} \label{cor-subisoexpexp}
    Let $\mathcal{G}$ be a graph class of single-exponential expansion.
    Then \textsc{Subgraph Isomorphism} on $\mathcal{G}$ can be solved in $2^{t^{O(1)}} \cdot n + O(n^4)$ time.
\end{corollary}
\begin{proof}
Let $(G,F)$ be an instance of \textsc{Subgraph Isomorphism} where $G \in \mathcal{G}$, $|V(G)| = n$, and $|V(F)| = t$.
As $\mathcal{G}$ is of single-exponential expansion, we have $\nabla_r(G) = 2^{r^{O(1)}}$ for $r \in \mathbb{N}$.
We use Lemma~\ref{lem-ordering} to compute the ordering $\sigma$ satisfying $\textnormal{wcol}_t(G,\sigma) \leq (7t \cdot \nabla_t(G))^{3t^2} = 2^{t^{O(1)}}$.
Now we apply Theorem~\ref{thm-subtwbranch} to solve the instance $(G,F)$ in $(2^{b_t(G)}+\text{wcol}_t(G,\sigma))^{O(t)} \cdot n$ time, i.e., $2^{t^{O(1)}} \cdot n$ time.
The overall running time is then $2^{t^{O(1)}} \cdot n + O(n^4)$.
\end{proof}

\subsection{Generalized subgraph isomorphism}

In our branching algorithm for \textsc{$\mathcal{F}$-Hitting} in Section~\ref{sec-branching}, we need a slightly more general version of \textsc{Subgraph Isomorphism}, in which we can have additional requirements for the subgraph we are looking for.
In this section, we discuss this generalization of \textsc{Subgraph Isomorphism} and show how to extend our algorithm to this setting.
We first define the problem.

\begin{tcolorbox}[colback=gray!5!white,colframe=gray!75!black]
        \textsc{Generalized Subgraph Isomorphism} \hfill \textbf{Parameter:} $t$
        \vspace{0.1cm} \\
        \textbf{Input:} A graph $G$ of $n$ vertices (taken from some graph class $\mathcal{G}$) and a graph $F$ of $t$ vertices together with a set $R_v \subseteq V(G)$ associated with each $v \in V(F)$.
        \vspace{0.1cm} \\
        %\textbf{Goal:} Compute a subgraph $H' \subseteq G$ and an isomorphism $f: V(H) \rightarrow V(H')$ between $H$ and $H'$ such that $f(v) \in R_v$ for all $v \in V(H)$.
        \textbf{Goal:} Find an $F$-copy $(H,\pi)$ in $G$ such that $\pi^{-1}(v) \in R_v$ for all $v \in V(F)$.
\end{tcolorbox}

For a vertex $v \in V(F)$, we call the set $R_v$ in the input the \textit{range} of $v$.
Compared to the standard problem, the only difference of \textsc{Generalized Subgraph Isomorphism} is that, in the isomorphism we find, every vertex $v \in V(F)$ must correspond to a vertex in its range $R_v$.

It turns out that our algorithm discussed in the previous sections directly extends to \textsc{Generalized Subgraph Isomorphism}, with only one change: redefining the relation $\simeq_X$.
Consider an instance $(G,F,\{R_v: v \in V(F)\})$ of the problem.
For every $u \in V(G)$, define $P_u = \{v \in V(F): u \in R_v\}$.
For two subgraphs $H,H' \subseteq G$ and a subset $X \subseteq V(G)$, we write $H \simeq_X H'$ if there exists an isomorphism $\pi: V(H) \rightarrow V(H')$ between $H$ and $H'$ such that $\pi(x) = x$ for all $x \in V(H) \cap X$, $\pi^{-1}(x) = x$ for all $x \in V(H') \cap X$, and in addition, $P_u = P_{\pi(u)}$ for all $u \in V(H)$.
We write $H \simeq H'$ if $H \simeq_\emptyset H'$.
Now we run Algorithm~\ref{alg-subiso} with $G$ and $t$ (ignoring $F$ at this point), using this new definition of $\simeq_X$.
The same analysis as in Section~\ref{sec-subisoana} shows that the algorithm returns a subgraph list $\mathcal{S}$ of $G$ satisfying that for any subgraph $H \subseteq G$ with $|V(F)| \leq t$, there exists $H' \in \mathcal{S}$ with $H' \simeq H$ (under the new definition).

\begin{observation}
    Let $(H,\pi)$ be an $F$-copy in $G$ such that $\pi^{-1}(v) \in R_v$ for all $v \in V(F)$, and $H' \subseteq G$ be a subgraph satisfying $H' \simeq H$ (under the new definition).
    Then there exists an isomorphism $\phi:V(H') \rightarrow V(F)$ between $H'$ and $F$ such that $\phi^{-1}(v) \in R_v$ for all $v \in V(F)$.
    %There exists an $F$-copy $(H,\pi)$ in $G$ such that $\pi^{-1}(v) \in R_v$ for all $v \in V(F)$ iff there exists $H' \in \mathcal{S}$ with an isomorphism $\phi:V(H') \rightarrow V(F)$ such that $\phi^{-1}(v) \in R_v$ for all $v \in V(F)$.
\end{observation}
\begin{proof}
Since $H' \simeq H$, there exists an isomorphism $\pi':V(H') \rightarrow V(H)$ between $H'$ and $H$ such that $P_{v} = P_{\pi'(v)}$ for all $v \in V(H')$.
We define $\phi = \pi \circ \pi'$, which is an isomorphism between $H'$ and $F$.
To see $\phi$ satisfies the desired condition, consider a vertex $v \in V(F)$.
We have $\phi^{-1}(v) = (\pi')^{-1}(\pi^{-1}(v))$.
By assumption, $\pi^{-1}(v) \in R_v$ and thus $v \in P_{\pi^{-1}(v)}$.
Furthermore, by the construction of $\pi'$, we have $P_{\pi^{-1}(v)} = P_{(\pi')^{-1}(\pi^{-1}(v))} = P_{\phi^{-1}(v)}$.
Therefore, $v \in P_{\phi^{-1}(v)}$ and thus $\phi^{-1}(v) \in R_v$.
\end{proof}

By the above observation, after we compute $\mathcal{S}$, we only need to compare $F$ with every $H \in \mathcal{S}$ and check if there exists an isomorphism $\phi:V(H) \rightarrow V(F)$ between $H'$ and $F$ satisfying $\phi^{-1}(v) \in R_v$ for all $v \in V(F)$.
If we successfully find $H$ and $\phi$, then we solve the instance because $(H,\phi)$ is the $F$-copy we want.
Otherwise, we know that $G$ does not contain any $F$-copy satisfying the desired condition, by the above observation.
The time cost for this step is $t^{O(t)} \cdot |\mathcal{S}|$.

Next, we bound the size of $\mathcal{S}$ and the time cost for computing $\mathcal{S}$.
Compared to the analysis in Section~\ref{sec-subisoana}, the only difference here is that the new relation $\simeq_X$ can partition a collection of subgraphs of $G$ into more equivalence classes, and thus slightly increase the time cost of the sub-routine \textsc{Rep} (as well as the size of $\mathcal{S}$).
We show the following analogy of Observation~\ref{obs-rep}, where the bounds are slightly different.

\begin{observation} \label{obs-rep'}
    $\textsc{Rep}(\mathcal{A},X,q)$ can be implemented in $(2^t+2^{b_p(G)}+q+|X|)^{O(p)} \cdot |\mathcal{A}|$ time and returns a collection of size $(2^t+2^{b_p(G)}+q +|X|)^{O(p)}$, where $p = \max_{A \in \mathcal{A}} |V(A)|$.
\end{observation}
\begin{proof}
We bound the number of equivalence classes $\mathcal{A}$ has for the new equivalence relation $\simeq_X$.
Everything else will be exactly the same as in the proof of Observation~\ref{obs-rep}.
Suppose $X = \{v_1,\dots,v_r\}$.
For each graph $A \in \mathcal{A}$, we make it as a labeled graph with labels in $(\{0\} \cup [r]) \times 2^{V(F)}$ by assigning to a vertex $v \in V(A)$ the label $(i,P_v)$ for $i \in [r]$ if $v = v_i$ and the label $(0,P_v)$ if $v \notin X$.
Then two graphs in $\mathcal{A}$ belong to the same equivalence class for $\simeq_X$ iff they are isomorphic as labeled graphs.
Note that $|E(A)| \leq b_p(G) \cdot p$ for all $A \in \mathcal{A}$.
Let $\mathcal{G}_{p,r,F}$ be the collection consisting of all different (up to isomorphism) labeled graphs of at most $p$ vertices and at most $b_p(G) \cdot p$ edges with label set $(\{0\} \cup [r]) \times 2^{V(F)}$.
The size of $\mathcal{G}_{p,r,F}$ is bounded by $(2^t r)^{O(p)} \cdot 2^{O(b_p(G) \cdot p)}$, so is the number of equivalence classes in $\mathcal{A}$.
The procedure of partitioning $\mathcal{A}$ into equivalence classes and computing the representative sets is exactly the same as in the proof of Observation~\ref{obs-rep}.
Plugging in the new bound on the number of equivalence classes, we see that $\textsc{Rep}(\mathcal{A},X,q)$ takes $(2^t+2^{b_p(G)}+q+r)^{O(p)} \cdot |\mathcal{A}|$ time and returns a collection of size $(2^t+2^{b_p(G)}+q+r)^{O(p)}$.
\end{proof}

Since $b_t(G) \leq t$, Observation~\ref{obs-rep'} implies that the call $\textsc{Rep}(\mathcal{S}_v,W_v,t)$ in line~6 takes $(2^t+|W_v|)^{O(t)} \cdot n$ time and returns a collection of size $(2^t+|W_v|)^{O(t)}$.
Therefore, the time cost for computing $\mathcal{S}$ is $(2^t+\text{wcol}_t(G,\sigma))^{O(t)} \cdot n$, which is also the overall running time of our algorithm (provided the ordering $\sigma$).
Based on this, we can obtain the following generalization of Corollary~\ref{cor-subisopolyexp} (with exactly the same proof).
We phrase it in a slightly different way for future use.

\begin{corollary} \label{cor-generalized}
    %Let $\mathcal{G}$ be a graph class admitting $(\eta,0,\rho)$-separators where $\rho < 1$.
    Let $\mathcal{G} \subseteq \mathcal{G}(\eta,0,\rho)$ where $\eta \geq 0$ and $\rho < 1$.
    Given a graph $G \in \mathcal{G}$ of $n$ vertices, after a preprocessing with $\eta^{O(1)} \cdot n^4$ time, one can solve any instance $(G,F,\{R_v: v \in V(F)\})$ of \textsc{Generalized Subgraph Isomorphism} in $(\eta t)^{O(t^3)} \cdot n$ time, where $t = |V(F)|$.
    The constants hidden in $O(\cdot)$ only depend on $\rho$.
\end{corollary}
